Measurements of normalized differential cross-sections for ttbar production in pp collisions at sqrt(s) = 7 TeV using the ATLAS detector

Measurements of normalized differential cross-sections for top-quark pair production are presented as a function of the top-quark transverse momentum, and of the mass, transverse momentum, and rapidity of the ttbar system, in proton--proton collisions at a center-of-mass energy of sqrt(s) = 7 TeV. The dataset corresponds to an integrated luminosity of 4.6 fb^-1, recorded in 2011 with the ATLAS detector at the CERN Large Hadron Collider. Events are selected in the lepton+jets channel, requiring exactly one lepton and at least four jets with at least one of the jets tagged as originating from a b-quark. The measured spectra are corrected for detector efficiency and resolution effects and are compared to several Monte Carlo simulations and theory calculations. The results are in fair agreement with the predictions in a wide kinematic range. Nevertheless, data distributions are softer than predicted for higher values of the mass of the ttbar system and of the top-quark transverse momentum. The measurements can also discriminate among different sets of parton distribution functions.

==> correlationMatrices.tex <==
\begin{table*} [!ht]
\footnotesize
\begin{center}

%%%
%%% keep this order: hadronic pTt, Mtt, pTtt, |ytt|
%%%
%%% cd yourdir/INT_XS_ttbar_diff/figures/correlationMatrices
%%% including stat correlations:
%%% cat correlationMatrices_Tag1_Top2_lhood_norm.tex correlationMatrices_Tag1_SystemMass_norm.tex correlationMatrices_Tag1_SystemPt_norm.tex correlationMatrices_Tag1_SystemAbsRap_norm.tex | grep -v caption | grep -v table | grep -v label | grep -v centering | grep -v foot

%%% without stat correlations: -- those to go here!
%%% cat correlationMatrices_Tag1_Top2_lhood_noStat_norm.tex correlationMatrices_Tag1_SystemMass_noStat_norm.tex correlationMatrices_Tag1_SystemPt_noStat_norm.tex correlationMatrices_Tag1_SystemAbsRap_noStat_norm.tex | grep -v caption | grep -v table | grep -v label | grep -v centering | grep -v foot

\noindent\makebox[\textwidth]{
\begin{tabular}{r| c c c c c c c}
\hline
{$\ptt{}$ [GeV]} & \multicolumn{1}{|c}{$[0, 50]$} & \multicolumn{1}{c}{$[50, 100]$} & \multicolumn{1}{c}{$[100, 150]$} & \multicolumn{1}{c}{$[150, 200]$} & \multicolumn{1}{c}{$[200, 250]$} & \multicolumn{1}{c}{$[250, 350]$} & \multicolumn{1}{|c}{$[350, 800]$} \\ 
\hline
        $[0,         50]$ &     1.00 &     0.49 &    -0.65 &    -0.75 &    -0.44 &    -0.03 &     0.21 \\ 
        $[50,        100]$ &     0.49 &     1.00 &    -0.44 &    -0.49 &    -0.71 &    -0.60 &    -0.39 \\ 
        $[100,        150]$ &    -0.65 &    -0.44 &     1.00 &     0.06 &    -0.12 &    -0.31 &    -0.22 \\ 
        $[150,        200]$ &    -0.75 &    -0.49 &     0.06 &     1.00 &     0.79 &     0.33 &    -0.09 \\ 
        $[200,        250]$ &    -0.44 &    -0.71 &    -0.12 &     0.79 &     1.00 &     0.75 &     0.29 \\ 
        $[250,        350]$ &    -0.03 &    -0.60 &    -0.31 &     0.33 &     0.75 &     1.00 &     0.78 \\ 
        $[350,        800]$ &     0.21 &    -0.39 &    -0.22 &    -0.09 &     0.29 &     0.78 &     1.00 \\ 
\hline
\end{tabular}}

\noindent\makebox[\textwidth]{
\begin{tabular}{r| c c c c c}
\hline
{$\mttbar{}$ [GeV]} & \multicolumn{1}{|c}{$[250, 450]$} & \multicolumn{1}{c}{$[450, 550]$} & \multicolumn{1}{c}{$[550, 700]$} & \multicolumn{1}{c}{$[700, 950]$} & \multicolumn{1}{|c}{$[950, 2700]$} \\ 
\hline
        $[250,        450]$ &     1.00 &    -0.89 &    -0.91 &    -0.40 &    -0.24 \\ 
        $[450,        550]$ &    -0.89 &     1.00 &     0.84 &     0.01 &    -0.14 \\ 
        $[550,        700]$ &    -0.91 &     0.84 &     1.00 &     0.12 &    -0.04 \\ 
        $[700,        950]$ &    -0.40 &     0.01 &     0.12 &     1.00 &     0.94 \\ 
        $[950,       2700]$ &    -0.24 &    -0.14 &    -0.04 &     0.94 &     1.00 \\ 
\hline
\end{tabular}}

\noindent\makebox[\textwidth]{
\begin{tabular}{r| c c c c}
\hline
{$\ptttbar{}$ [GeV]} & \multicolumn{1}{|c}{$[0, 40]$} & \multicolumn{1}{c}{$[40, 170]$} & \multicolumn{1}{c}{$[170, 340]$} & \multicolumn{1}{|c}{$[340, 1000]$} \\ 
\hline
        $[0,         40]$ &     1.00 &    -0.99 &    -0.86 &    -0.53 \\ 
        $[40,        170]$ &    -0.99 &     1.00 &     0.78 &     0.46 \\ 
        $[170,        340]$ &    -0.86 &     0.78 &     1.00 &     0.70 \\ 
        $[340,       1000]$ &    -0.53 &     0.46 &     0.70 &     1.00 \\ 
\hline
\end{tabular}}

\noindent\makebox[\textwidth]{
\begin{tabular}{r| c c c}
\hline
{$\absyttbar{}$ } & \multicolumn{1}{|c}{$[0, 0.5]$} & \multicolumn{1}{c}{$[0.5, 1]$} & \multicolumn{1}{|c}{$[1, 2.5]$} \\ 
\hline
        $[0,        0.5]$ &     1.00 &     0.90 &    -0.99 \\ 
        $[0.5,          1]$ &     0.90 &     1.00 &    -0.94 \\ 
        $[1,        2.5]$ &    -0.99 &    -0.94 &     1.00 \\ 
\hline
\end{tabular}}



\caption{Bin-wise systematic correlation matrices for the normalized differential cross-sections. From top to bottom: top quark $\pt$; and mass, $\pt$ and the absolute value of the rapidity of the $\ttbar$ system.}
\label{tab:Corr}
\end{center}
\end{table*}



==> relativeUncertaintiesInCombination_Tag1_SystemAbsRap_Norm.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dabsyttbar}$ Uncertainties [\%] &    [0.0, 0.5] &    [0.5, 1.0] &    [1.0, 2.5] \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  -0.05 }_{  -0.08}$ & $^{  -0.13 }_{  -0.03}$ & $^{  +0.05 }_{  +0.09}$ \\ [0.5mm] 
Closeby jets (JES) & $^{  -0.24 }_{  +0.07}$ & $^{  -0.06 }_{  -0.02}$ & $^{  +0.36 }_{  -0.11}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  -0.14 }_{  +0.08}$ & $^{  -0.02 }_{  -0.01}$ & $^{  +0.20 }_{  -0.14}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  +0.00 }_{  +0.00}$ & $^{  -0.03 }_{  -0.02}$ & $^{  -0.01 }_{  -0.03}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  -0.07 }_{  -0.02}$ & $^{  -0.05 }_{  -0.04}$ & $^{  +0.16 }_{  +0.02}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  -0.10 }_{  +0.01}$ & $^{  -0.07 }_{  +0.01}$ & $^{  +0.16 }_{  -0.02}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  -0.07 }_{  -0.00}$ & $^{  -0.03 }_{  -0.06}$ & $^{  +0.11 }_{  -0.02}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  -0.01 }_{  -0.03}$ & $^{  -0.06 }_{  -0.03}$ & $^{  -0.03 }_{  +0.03}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  +0.01 }_{  -0.02}$ & $^{  +0.02 }_{  -0.02}$ & $^{  -0.03 }_{  +0.00}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  -0.03 }_{  -0.03}$ & $^{  -0.07 }_{  -0.06}$ & $^{  +0.07 }_{  +0.05}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  -0.05 }_{  +0.03}$ & $^{  -0.05 }_{  +0.02}$ & $^{  +0.07 }_{  -0.08}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  -0.07 }_{  -0.03}$ & $^{  -0.05 }_{  -0.03}$ & $^{  +0.12 }_{  +0.07}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  -0.09 }_{  -0.03}$ & $^{  -0.07 }_{  -0.05}$ & $^{  +0.12 }_{  +0.07}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  -0.69 }_{  +0.45}$ & $^{  -0.10 }_{  -0.06}$ & $^{  +1.06 }_{  -0.73}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  -0.13 }_{  -0.01}$ & $^{  -0.07 }_{  -0.03}$ & $^{  +0.19 }_{  -0.02}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  -0.08 }_{  -0.04}$ & $^{  -0.05 }_{  -0.06}$ & $^{  +0.10 }_{  +0.08}$ \\ [0.5mm] 
Flavor response (JES) & $^{  -0.01 }_{  +0.05}$ & $^{  -0.02 }_{  -0.11}$ & $^{  -0.04 }_{  -0.11}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  -0.12 }_{  -0.04}$ & $^{  -0.03 }_{  -0.10}$ & $^{  +0.19 }_{  +0.10}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  -0.02 }_{  +0.02}$ & $^{  +0.03 }_{  +0.03}$ & $^{  +0.02 }_{  -0.08}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  -0.15 }_{  +0.11}$ & $^{  -0.09 }_{  -0.00}$ & $^{  +0.27 }_{  -0.22}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  -0.01 }_{  -0.01}$ & $^{  +0.00 }_{  +0.00}$ & $^{  +0.02 }_{  +0.03}$ \\ [0.5mm] 
JES uncertainty in background & $^{  +0.01 }_{  +0.31}$ & $^{  -0.02 }_{  +0.11}$ & $^{  -0.14 }_{  -0.56}$ \\ [0.5mm] 
Jet energy resolution & $^{  +0.28 }_{  -0.28}$ & $^{  +0.17 }_{  -0.17}$ & $^{  -0.62 }_{  +0.62}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  +0.00 }_{  -0.00}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.02 }_{  +0.02}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  +0.01 }_{  +0.00}$ & $^{  -0.01 }_{  +0.02}$ & $^{  -0.03 }_{  -0.00}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  -0.02 }_{  +0.02}$ & $^{  +0.00 }_{  +0.00}$ & $^{  +0.01 }_{  -0.01}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  -0.01 }_{  +0.01}$ & $^{  +0.01 }_{  -0.01}$ & $^{  +0.03 }_{  -0.04}$ \\ [0.5mm] 
$e$ energy resolution & $^{  +0.06 }_{  +0.01}$ & $^{  +0.00 }_{  +0.02}$ & $^{  -0.13 }_{  -0.02}$ \\ [0.5mm] 
$e$ energy scale & $^{  -0.04 }_{  -0.03}$ & $^{  -0.06 }_{  -0.01}$ & $^{  +0.04 }_{  +0.05}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  -0.00 }_{  -0.00}$ & $^{  -0.04 }_{  -0.06}$ & $^{  -0.00 }_{  +0.01}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  +0.00 }_{  +0.00}$ & $^{  +0.01 }_{  +0.05}$ & $^{  -0.04 }_{  -0.05}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  -0.00 }_{  +0.00}$ & $^{  +0.00 }_{  -0.00}$ & $^{  +0.07 }_{  -0.07}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  -0.05 }_{  +0.05}$ & $^{  -0.02 }_{  +0.02}$ & $^{  +0.11 }_{  -0.11}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  +0.07 }_{  -0.07}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.14 }_{  +0.14}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  -0.01 }_{  +0.01}$ & $^{  -0.03 }_{  +0.03}$ & $^{  +0.05 }_{  -0.05}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  -0.05 }_{  +0.06}$ & $^{  -0.13 }_{  -0.01}$ & $^{  +0.14 }_{  -0.21}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  +0.03 }_{  +0.05}$ & $^{  -0.12 }_{  -0.06}$ & $^{  -0.10 }_{  -0.14}$ \\ [0.5mm] 
MC generator & $^{  -1.29 }_{  +1.29}$ & $^{  -0.91 }_{  +0.91}$ & $^{  +3.75 }_{  -3.75}$ \\ [0.5mm] 
Fragmentation & $^{  -1.60 }_{  +1.60}$ & $^{  -0.44 }_{  +0.44}$ & $^{  +3.99 }_{  -3.99}$ \\ [0.5mm] 
IFSR & $^{  -0.30 }_{  +0.30}$ & $^{  -0.03 }_{  +0.03}$ & $^{  +0.30 }_{  -0.30}$ \\ [0.5mm] 
PDF & $^{  -1.17 }_{  +1.17}$ & $^{  -0.13 }_{  +0.13}$ & $^{  +2.05 }_{  -2.05}$ \\ [0.5mm] 
MC statistics & $^{  +0.20 }_{  -0.20}$ & $^{  +0.03 }_{  -0.03}$ & $^{  +0.29 }_{  -0.29}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  -0.05 }_{  +0.05}$ & $^{  +0.03 }_{  +0.00}$ & $^{  +0.07 }_{  -0.08}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  -0.05 }_{  -0.00}$ & $^{  +0.03 }_{  -0.03}$ & $^{  +0.07 }_{  +0.01}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  -0.19 }_{  +0.18}$ & $^{  +0.05 }_{  -0.04}$ & $^{  +0.25 }_{  -0.25}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  -0.04 }_{  +0.04}$ & $^{  -0.00 }_{  +0.00}$ & $^{  +0.10 }_{  -0.10}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  +0.02 }_{  -0.02}$ & $^{  -0.01 }_{  +0.00}$ & $^{  -0.02 }_{  +0.01}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  +0.02 }_{  -0.01}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.02 }_{  +0.00}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  -0.04 }_{  +0.05}$ & $^{  +0.03 }_{  -0.03}$ & $^{  +0.07 }_{  -0.09}$ \\ [0.5mm] 
Multijet normalization & $^{  -0.23 }_{  +0.22}$ & $^{  -0.05 }_{  +0.05}$ & $^{  +0.48 }_{  -0.48}$ \\ [0.5mm] 
Multijet shape & $^{  -0.17 }_{  +0.16}$ & $^{  -0.03 }_{  +0.01}$ & $^{  +0.36 }_{  -0.36}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  -0.15 }_{  +0.15}$ & $^{  -0.05 }_{  +0.05}$ & $^{  +0.28 }_{  -0.28}$ \\ [0.5mm] 
Dilepton background normalization & $^{  +0.01 }_{  -0.01}$ & $^{  +0.01 }_{  -0.01}$ & $^{  -0.02 }_{  +0.02}$ \\ [0.5mm] 
\hline
Channels BLUE weights  & (1.05 ,-0.05) & (-1.89 ,2.89) & (1.44 ,-0.44) \\ [2mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemAbsRap_Norm_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dabsyttbar}$ Uncertainties [\%] &    [0.0, 0.5] &    [0.5, 1.0] &    [1.0, 2.5] \\ 
\hline
\hline
Jet energy scale & $^{+    0.8 }_{-    0.6}$ & $^{+    0.3 }_{-    0.2}$ & $^{+    1.3 }_{-    1.0}$ \\ [1mm] 
Jet energy resolution & $\pm    0.3$ & $\pm    0.2$ & $\pm    0.6$ \\ [1mm] 
Jet reconstruction efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
$b$-quark tagging efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
$c$-quark tagging efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Light-jet tagging efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Lepton selection and scaling & $\pm    0.1$ & ${\rm --}$ & $\pm    0.2$ \\ [1mm] 
\Etmiss{} cell-out & $^{\rm --}_{-\rm --}$ & $^{+    0.1 }_{-\rm --}$ & $^{+    0.1 }_{-    0.2}$ \\ [1mm] 
\Etmiss{} pile-up & $^{\rm --}_{-\rm --}$ & $\pm    0.1$ & $\pm    0.1$ \\ [1mm] 
MC generator & $\pm    1.3$ & $\pm    0.9$ & $\pm    3.8$ \\ [1mm] 
Fragmentation & $\pm    1.6$ & $\pm    0.4$ & $\pm    4.0$ \\ [1mm] 
IFSR & $\pm    0.3$ & ${\rm --}$ & $\pm    0.3$ \\ [1mm] 
PDF & $\pm    1.2$ & $\pm    0.1$ & $\pm    2.0$ \\ [1mm] 
MC statistics & $\pm    0.2$ & ${\rm --}$ & $\pm    0.3$ \\ [1mm] 
\Wboson+jets & $\pm    0.2$ & ${\rm --}$ & $\pm    0.3$ \\ [1mm] 
Other backgrounds & $\pm    0.3$ & ${\rm --}$ & $\pm    0.7$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$0.9 & $\pm$0.8 & $\pm$1.8 \\ [2mm] 
 Total systematic uncertainty  & $^{+    2.6 }_{-    2.5}$ & $\pm    1.1$ & $^{+    6.1 }_{-    6.0}$ \\ [2mm] 
\hline
%%%Channels BLUE weights  & (1.05 ,-0.05) & (-1.89 ,2.89) & (1.44 ,-0.44) \\ [2mm] 
\hline
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemMass_Norm.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dmttbar} $ Uncertainties [\%] $/$ Bins [GeV] &    [250, 450] &    [450, 550] &    [550, 700] &    [700, 950] &    [950,2700] \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  -0.37 }_{  +0.58}$ & $^{  +0.25 }_{  -0.39}$ & $^{  +0.44 }_{  -0.80}$ & $^{  +0.47 }_{  -0.78}$ & $^{  +0.52 }_{  -0.80}$ \\ [0.5mm] 
Closeby jets (JES) & $^{  -0.47 }_{  +0.42}$ & $^{  +0.25 }_{  -0.25}$ & $^{  +0.74 }_{  -0.64}$ & $^{  +0.89 }_{  -0.98}$ & $^{  +1.12 }_{  -1.41}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  -0.69 }_{  +0.54}$ & $^{  +0.40 }_{  -0.34}$ & $^{  +1.00 }_{  -0.70}$ & $^{  +1.42 }_{  -0.99}$ & $^{  +1.67 }_{  -1.06}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  -0.08 }_{  -0.03}$ & $^{  +0.06 }_{  -0.00}$ & $^{  +0.11 }_{  +0.07}$ & $^{  +0.19 }_{  +0.15}$ & $^{  +0.22 }_{  +0.16}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  -0.05 }_{  -0.02}$ & $^{  -0.02 }_{  -0.02}$ & $^{  +0.11 }_{  +0.09}$ & $^{  +0.20 }_{  +0.01}$ & $^{  +0.22 }_{  +0.00}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  +0.01 }_{  -0.05}$ & $^{  +0.02 }_{  +0.00}$ & $^{  -0.00 }_{  +0.12}$ & $^{  +0.02 }_{  +0.17}$ & $^{  +0.02 }_{  +0.27}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  -0.20 }_{  +0.05}$ & $^{  +0.33 }_{  -0.21}$ & $^{  +0.25 }_{  +0.04}$ & $^{  -0.34 }_{  +0.24}$ & $^{  -0.75 }_{  +0.44}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  -0.31 }_{  +0.14}$ & $^{  +0.18 }_{  -0.07}$ & $^{  +0.48 }_{  -0.21}$ & $^{  +0.60 }_{  -0.32}$ & $^{  +0.65 }_{  -0.33}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  +0.23 }_{  -0.32}$ & $^{  -0.07 }_{  +0.14}$ & $^{  -0.32 }_{  +0.47}$ & $^{  -0.49 }_{  +0.66}$ & $^{  -0.43 }_{  +0.69}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  -0.08 }_{  +0.05}$ & $^{  +0.02 }_{  -0.10}$ & $^{  +0.16 }_{  -0.03}$ & $^{  +0.19 }_{  +0.02}$ & $^{  +0.16 }_{  +0.10}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  +0.17 }_{  -0.20}$ & $^{  -0.10 }_{  -0.01}$ & $^{  -0.29 }_{  +0.39}$ & $^{  -0.38 }_{  +0.62}$ & $^{  -0.42 }_{  +0.86}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  -0.04 }_{  +0.02}$ & $^{  +0.02 }_{  +0.03}$ & $^{  +0.14 }_{  -0.06}$ & $^{  +0.04 }_{  -0.05}$ & $^{  -0.02 }_{  +0.07}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  -0.13 }_{  +0.13}$ & $^{  +0.03 }_{  -0.07}$ & $^{  +0.19 }_{  -0.15}$ & $^{  +0.32 }_{  -0.28}$ & $^{  +0.41 }_{  -0.26}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  -0.80 }_{  +0.78}$ & $^{  +0.36 }_{  -0.39}$ & $^{  +1.22 }_{  -1.07}$ & $^{  +1.78 }_{  -1.80}$ & $^{  +2.02 }_{  -2.29}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  -0.11 }_{  +0.00}$ & $^{  +0.13 }_{  -0.05}$ & $^{  +0.17 }_{  +0.04}$ & $^{  +0.11 }_{  +0.08}$ & $^{  +0.09 }_{  +0.15}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  -0.05 }_{  +0.08}$ & $^{  -0.08 }_{  -0.06}$ & $^{  +0.14 }_{  -0.04}$ & $^{  +0.32 }_{  -0.31}$ & $^{  +0.36 }_{  -0.45}$ \\ [0.5mm] 
Flavor response (JES) & $^{  +0.04 }_{  -0.08}$ & $^{  -0.06 }_{  -0.09}$ & $^{  -0.05 }_{  +0.21}$ & $^{  +0.06 }_{  +0.36}$ & $^{  +0.18 }_{  +0.50}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  -0.05 }_{  +0.05}$ & $^{  +0.02 }_{  +0.03}$ & $^{  +0.21 }_{  -0.12}$ & $^{  -0.08 }_{  -0.24}$ & $^{  -0.26 }_{  -0.44}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  +0.07 }_{  -0.10}$ & $^{  -0.01 }_{  -0.04}$ & $^{  -0.06 }_{  +0.11}$ & $^{  -0.31 }_{  +0.41}$ & $^{  -0.47 }_{  +0.54}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  -0.19 }_{  +0.08}$ & $^{  +0.06 }_{  -0.01}$ & $^{  +0.32 }_{  -0.07}$ & $^{  +0.35 }_{  -0.25}$ & $^{  +0.32 }_{  -0.39}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  -0.00 }_{  -0.00}$ & $^{  +0.01 }_{  +0.01}$ & $^{  -0.00 }_{  -0.00}$ & $^{  -0.02 }_{  -0.01}$ & $^{  -0.03 }_{  -0.01}$ \\ [0.5mm] 
JES uncertainty in background & $^{  +0.09 }_{  -0.07}$ & $^{  -0.15 }_{  +0.09}$ & $^{  -0.03 }_{  +0.12}$ & $^{  -0.02 }_{  -0.23}$ & $^{  +0.33 }_{  -0.60}$ \\ [0.5mm] 
Jet energy resolution & $^{  -0.33 }_{  +0.33}$ & $^{  +0.39 }_{  -0.39}$ & $^{  +0.28 }_{  -0.28}$ & $^{  +0.61 }_{  -0.61}$ & $^{  +0.87 }_{  -0.87}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  +0.00 }_{  -0.00}$ & $^{  +0.05 }_{  -0.05}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.01 }_{  +0.01}$ & $^{  +0.00 }_{  -0.00}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  -0.97 }_{  +0.76}$ & $^{  +0.41 }_{  -0.38}$ & $^{  +1.53 }_{  -1.19}$ & $^{  +2.02 }_{  -1.37}$ & $^{  +2.18 }_{  -1.30}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  +0.05 }_{  -0.05}$ & $^{  -0.05 }_{  +0.05}$ & $^{  -0.08 }_{  +0.08}$ & $^{  +0.00 }_{  +0.01}$ & $^{  +0.04 }_{  -0.03}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  +0.02 }_{  -0.02}$ & $^{  -0.05 }_{  +0.05}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.07 }_{  +0.07}$ \\ [0.5mm] 
$e$ energy resolution & $^{  +0.04 }_{  +0.02}$ & $^{  +0.00 }_{  -0.00}$ & $^{  -0.06 }_{  -0.04}$ & $^{  -0.09 }_{  -0.06}$ & $^{  -0.16 }_{  -0.07}$ \\ [0.5mm] 
$e$ energy scale & $^{  +0.08 }_{  +0.05}$ & $^{  -0.02 }_{  -0.01}$ & $^{  -0.09 }_{  -0.07}$ & $^{  -0.13 }_{  +0.00}$ & $^{  -0.18 }_{  +0.06}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  +0.01 }_{  +0.06}$ & $^{  -0.02 }_{  -0.09}$ & $^{  +0.04 }_{  -0.13}$ & $^{  -0.05 }_{  +0.05}$ & $^{  -0.09 }_{  +0.27}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  +0.10 }_{  +0.06}$ & $^{  +0.01 }_{  +0.02}$ & $^{  -0.16 }_{  -0.13}$ & $^{  -0.34 }_{  -0.20}$ & $^{  -0.43 }_{  -0.24}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  -0.05 }_{  +0.05}$ & $^{  +0.04 }_{  -0.04}$ & $^{  +0.13 }_{  -0.13}$ & $^{  +0.01 }_{  -0.01}$ & $^{  +0.03 }_{  -0.03}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  +0.02 }_{  -0.02}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.02 }_{  +0.03}$ & $^{  -0.01 }_{  +0.01}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  +0.01 }_{  -0.01}$ & $^{  -0.00 }_{  +0.00}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.06 }_{  +0.05}$ & $^{  -0.07 }_{  +0.07}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  +0.03 }_{  -0.03}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.05 }_{  +0.05}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.09 }_{  +0.09}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  +0.07 }_{  +0.06}$ & $^{  -0.01 }_{  +0.11}$ & $^{  -0.05 }_{  -0.05}$ & $^{  -0.08 }_{  -0.33}$ & $^{  +0.04 }_{  -0.49}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  +0.02 }_{  -0.03}$ & $^{  -0.02 }_{  +0.01}$ & $^{  +0.09 }_{  +0.13}$ & $^{  +0.11 }_{  +0.02}$ & $^{  +0.10 }_{  -0.13}$ \\ [0.5mm] 
MC generator & $^{  -2.53 }_{  +2.53}$ & $^{  +2.21 }_{  -2.21}$ & $^{  +2.64 }_{  -2.64}$ & $^{  +2.84 }_{  -2.84}$ & $^{  +3.35 }_{  -3.35}$ \\ [0.5mm] 
Fragmentation & $^{  +0.29 }_{  -0.29}$ & $^{  +0.00 }_{  -0.00}$ & $^{  -0.55 }_{  +0.55}$ & $^{  -1.03 }_{  +1.03}$ & $^{  -0.63 }_{  +0.63}$ \\ [0.5mm] 
IFSR & $^{  +1.23 }_{  -1.23}$ & $^{  -0.83 }_{  +0.83}$ & $^{  -1.48 }_{  +1.48}$ & $^{  -0.49 }_{  +0.49}$ & $^{  -0.07 }_{  +0.07}$ \\ [0.5mm] 
PDF & $^{  -0.15 }_{  +0.15}$ & $^{  +0.02 }_{  -0.02}$ & $^{  +0.14 }_{  -0.14}$ & $^{  +0.35 }_{  -0.35}$ & $^{  +1.93 }_{  -1.93}$ \\ [0.5mm] 
MC statistics & $^{  +0.41 }_{  -0.41}$ & $^{  +0.41 }_{  -0.41}$ & $^{  +0.63 }_{  -0.63}$ & $^{  +1.01 }_{  -1.01}$ & $^{  +1.51 }_{  -1.51}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  -0.06 }_{  -0.01}$ & $^{  -0.06 }_{  +0.02}$ & $^{  +0.13 }_{  -0.00}$ & $^{  +0.43 }_{  -0.04}$ & $^{  +0.71 }_{  -0.14}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  -0.06 }_{  +0.07}$ & $^{  -0.06 }_{  +0.04}$ & $^{  +0.13 }_{  -0.12}$ & $^{  +0.43 }_{  -0.37}$ & $^{  +0.71 }_{  -0.55}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  -0.12 }_{  +0.11}$ & $^{  -0.05 }_{  +0.05}$ & $^{  +0.29 }_{  -0.27}$ & $^{  +0.57 }_{  -0.53}$ & $^{  +1.00 }_{  -0.92}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  +0.03 }_{  -0.03}$ & $^{  -0.09 }_{  +0.10}$ & $^{  -0.01 }_{  +0.02}$ & $^{  +0.32 }_{  -0.32}$ & $^{  +0.60 }_{  -0.61}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  +0.02 }_{  -0.05}$ & $^{  -0.01 }_{  +0.03}$ & $^{  -0.06 }_{  +0.08}$ & $^{  +0.02 }_{  +0.07}$ & $^{  +0.04 }_{  +0.09}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  +0.02 }_{  +0.03}$ & $^{  -0.01 }_{  -0.03}$ & $^{  -0.06 }_{  -0.02}$ & $^{  +0.02 }_{  -0.10}$ & $^{  +0.04 }_{  -0.14}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  -0.02 }_{  +0.03}$ & $^{  -0.05 }_{  +0.06}$ & $^{  +0.04 }_{  -0.06}$ & $^{  +0.31 }_{  -0.41}$ & $^{  +0.54 }_{  -0.69}$ \\ [0.5mm] 
Multijet normalization & $^{  +0.16 }_{  -0.17}$ & $^{  -0.16 }_{  +0.16}$ & $^{  -0.20 }_{  +0.21}$ & $^{  +0.61 }_{  -0.57}$ & $^{  +1.59 }_{  -1.52}$ \\ [0.5mm] 
Multijet shape & $^{  -0.10 }_{  +0.03}$ & $^{  +0.03 }_{  +0.06}$ & $^{  +0.09 }_{  +0.00}$ & $^{  +0.30 }_{  -0.84}$ & $^{  +0.60 }_{  -1.89}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  +0.06 }_{  -0.06}$ & $^{  -0.06 }_{  +0.06}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.02 }_{  +0.02}$ & $^{  +0.06 }_{  -0.06}$ \\ [0.5mm] 
Dilepton background normalization & $^{  +0.14 }_{  -0.13}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.22 }_{  +0.21}$ & $^{  -0.36 }_{  +0.34}$ & $^{  -0.40 }_{  +0.38}$ \\ [0.5mm] 
\hline
Channels BLUE weights  & (0.35 ,0.65) & (0.15 ,0.85) & (0.24 ,0.76) & (0.51 ,0.49) & (0.50 ,0.50) \\ [2mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemMass_Norm_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dmttbar} $ Uncertainties [\%] $/$ Bins [GeV] &    [250, 450] &    [450, 550] &    [550, 700] &    [700, 950] &    [950,2700] \\ 
\hline
\hline
Jet energy scale & $\pm    1.3$ & $\pm    0.8$ & $^{+    2.0 }_{-    1.8}$ & $^{+    2.8 }_{-    2.7}$ & $^{+    3.3 }_{-    3.5}$ \\ [1mm] 
Jet energy resolution & $\pm    0.3$ & $\pm    0.4$ & $\pm    0.3$ & $\pm    0.6$ & $\pm    0.9$ \\ [1mm] 
Jet reconstruction efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
$b$-quark tagging efficiency & $^{+    1.0 }_{-    0.8}$ & $\pm    0.4$ & $^{+    1.5 }_{-    1.2}$ & $^{+    2.0 }_{-    1.4}$ & $^{+    2.2 }_{-    1.3}$ \\ [1mm] 
$c$-quark tagging efficiency & $^{\rm --}_{-\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Light-jet tagging efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Lepton selection and scaling & $^{+    0.2 }_{-    0.1}$ & ${\rm --}$ & $\pm    0.2$ & $^{+    0.4 }_{-    0.2}$ & $^{+    0.5 }_{-    0.4}$ \\ [1mm] 
\Etmiss{} cell-out & ${\rm --}$ & $^{\rm --}_{-    0.1}$ & $^{\rm --}_{-\rm --}$ & $^{\rm --}_{-    0.3}$ & $^{\rm --}_{-    0.5}$ \\ [1mm] 
\Etmiss{} pile-up & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & $^{+    0.1 }_{-\rm --}$ & ${\rm --}$ \\ [1mm] 
MC generator & $\pm    2.5$ & $\pm    2.2$ & $\pm    2.6$ & $\pm    2.8$ & $\pm    3.3$ \\ [1mm] 
Fragmentation & $\pm    0.3$ & ${\rm --}$ & $\pm    0.5$ & $\pm    1.0$ & $\pm    0.6$ \\ [1mm] 
IFSR & $\pm    1.2$ & $\pm    0.8$ & $\pm    1.5$ & $\pm    0.5$ & ${\rm --}$ \\ [1mm] 
PDF & $\pm    0.2$ & ${\rm --}$ & $\pm    0.1$ & $\pm    0.3$ & $\pm    1.9$ \\ [1mm] 
MC statistics & $\pm    0.4$ & $\pm    0.4$ & $\pm    0.6$ & $\pm    1.0$ & $\pm    1.5$ \\ [1mm] 
\Wboson+jets & $^{+    0.2 }_{-    0.1}$ & $\pm    0.1$ & $^{+    0.4 }_{-    0.3}$ & $^{+    0.9 }_{-    0.8}$ & $^{+    1.6 }_{-    1.4}$ \\ [1mm] 
Other backgrounds & $\pm    0.2$ & $\pm    0.2$ & $\pm    0.3$ & $^{+    0.8 }_{-    1.1}$ & $^{+    1.7 }_{-    2.5}$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$0.9 & $\pm$1.1 & $\pm$1.6 & $\pm$2.6 & $\pm$4.0 \\ [2mm] 
 Total systematic uncertainty  & $\pm    3.3$ & $\pm    2.6$ & $^{+    4.1 }_{-    3.9}$ & $^{+    4.9 }_{-    4.7}$ & $^{+    6.3 }_{-    6.4}$ \\ [2mm] 
\hline
%%%Channels BLUE weights  & (0.35 ,0.65) & (0.15 ,0.85) & (0.24 ,0.76) & (0.51 ,0.49) & (0.50 ,0.50) \\ [2mm] 
\hline
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemPt_Norm.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptttbar}$ Uncertainties [\%] $/$ Bins [GeV] &    [0,  40] &    [40, 170] &    [170, 340] &    [340,1000] \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  -0.04 }_{  -0.02}$ & $^{  -0.12 }_{  +0.09}$ & $^{  +0.27 }_{  -0.54}$ & $^{  +0.21 }_{  -0.74}$ \\ [0.5mm] 
Closeby jets (JES) & $^{  -0.57 }_{  +0.64}$ & $^{  +0.73 }_{  -0.97}$ & $^{  +1.42 }_{  -1.21}$ & $^{  +1.37 }_{  -1.31}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  -0.49 }_{  +0.43}$ & $^{  +0.37 }_{  -0.26}$ & $^{  +1.86 }_{  -2.00}$ & $^{  +2.66 }_{  -3.06}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  +0.04 }_{  -0.04}$ & $^{  +0.01 }_{  +0.04}$ & $^{  -0.32 }_{  -0.06}$ & $^{  -0.69 }_{  -0.12}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  -0.07 }_{  +0.03}$ & $^{  +0.17 }_{  +0.05}$ & $^{  +0.13 }_{  -0.48}$ & $^{  +0.22 }_{  -1.05}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  +0.01 }_{  -0.01}$ & $^{  +0.07 }_{  +0.16}$ & $^{  -0.35 }_{  +0.08}$ & $^{  -0.75 }_{  -0.12}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  -0.53 }_{  +0.40}$ & $^{  +0.63 }_{  -0.51}$ & $^{  +0.82 }_{  -0.69}$ & $^{  +0.33 }_{  -0.52}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  -0.02 }_{  +0.20}$ & $^{  +0.13 }_{  -0.02}$ & $^{  +0.22 }_{  -0.90}$ & $^{  +0.26 }_{  -1.45}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  +0.11 }_{  -0.13}$ & $^{  -0.01 }_{  +0.29}$ & $^{  -0.53 }_{  +0.14}$ & $^{  -0.64 }_{  +0.11}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  -0.05 }_{  +0.06}$ & $^{  +0.08 }_{  +0.05}$ & $^{  +0.00 }_{  -0.28}$ & $^{  -0.07 }_{  -0.55}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  -0.16 }_{  +0.19}$ & $^{  +0.46 }_{  -0.22}$ & $^{  +0.45 }_{  -0.23}$ & $^{  +0.10 }_{  -0.00}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  +0.07 }_{  -0.01}$ & $^{  +0.00 }_{  +0.04}$ & $^{  -0.08 }_{  -0.12}$ & $^{  -0.21 }_{  -0.21}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  -0.09 }_{  +0.09}$ & $^{  +0.22 }_{  -0.07}$ & $^{  +0.20 }_{  -0.55}$ & $^{  +0.26 }_{  -0.93}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  -0.86 }_{  +0.93}$ & $^{  +0.91 }_{  -0.73}$ & $^{  +2.67 }_{  -2.55}$ & $^{  +3.29 }_{  -3.39}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  -0.15 }_{  +0.14}$ & $^{  +0.29 }_{  +0.05}$ & $^{  +0.26 }_{  -0.56}$ & $^{  -0.05 }_{  -1.03}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  -0.06 }_{  +0.08}$ & $^{  +0.18 }_{  -0.04}$ & $^{  +0.39 }_{  -0.38}$ & $^{  +0.44 }_{  -0.47}$ \\ [0.5mm] 
Flavor response (JES) & $^{  -0.31 }_{  +0.37}$ & $^{  +0.45 }_{  -0.29}$ & $^{  +0.63 }_{  -0.88}$ & $^{  +0.57 }_{  -1.13}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  -0.15 }_{  +0.10}$ & $^{  -0.02 }_{  -0.19}$ & $^{  +0.39 }_{  -0.47}$ & $^{  +0.44 }_{  -0.42}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  -0.04 }_{  +0.10}$ & $^{  +0.04 }_{  +0.13}$ & $^{  +0.04 }_{  -0.20}$ & $^{  -0.28 }_{  -0.63}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  -0.06 }_{  +0.12}$ & $^{  +0.37 }_{  -0.14}$ & $^{  +0.02 }_{  -0.51}$ & $^{  -0.31 }_{  -0.75}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  +0.03 }_{  +0.02}$ & $^{  -0.03 }_{  -0.03}$ & $^{  -0.09 }_{  -0.09}$ & $^{  -0.11 }_{  -0.11}$ \\ [0.5mm] 
JES uncertainty in background & $^{  -1.05 }_{  +0.95}$ & $^{  +1.15 }_{  -0.79}$ & $^{  +2.61 }_{  -2.05}$ & $^{  +3.78 }_{  -2.28}$ \\ [0.5mm] 
Jet energy resolution & $^{  +3.18 }_{  -3.18}$ & $^{  -3.67 }_{  +3.67}$ & $^{  -6.88 }_{  +6.88}$ & $^{  -7.82 }_{  +7.82}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  -0.07 }_{  +0.07}$ & $^{  +0.19 }_{  -0.19}$ & $^{  -0.06 }_{  +0.06}$ & $^{  -0.22 }_{  +0.22}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  -0.01 }_{  -0.10}$ & $^{  -0.01 }_{  +0.09}$ & $^{  +0.36 }_{  +0.16}$ & $^{  +1.00 }_{  -0.15}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  -0.09 }_{  +0.08}$ & $^{  +0.20 }_{  -0.19}$ & $^{  +0.35 }_{  -0.30}$ & $^{  +0.39 }_{  -0.33}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  +0.02 }_{  +0.00}$ & $^{  +0.07 }_{  -0.09}$ & $^{  +0.12 }_{  -0.15}$ & $^{  +0.19 }_{  -0.21}$ \\ [0.5mm] 
$e$ energy resolution & $^{  -0.07 }_{  -0.06}$ & $^{  +0.26 }_{  +0.27}$ & $^{  +0.19 }_{  -0.01}$ & $^{  +0.33 }_{  -0.15}$ \\ [0.5mm] 
$e$ energy scale & $^{  -0.03 }_{  +0.03}$ & $^{  +0.24 }_{  -0.04}$ & $^{  -0.46 }_{  -0.38}$ & $^{  -0.73 }_{  -0.66}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  -0.12 }_{  -0.00}$ & $^{  +0.04 }_{  +0.00}$ & $^{  -0.06 }_{  -0.03}$ & $^{  -0.26 }_{  -0.11}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  -0.01 }_{  -0.08}$ & $^{  +0.00 }_{  +0.02}$ & $^{  +0.06 }_{  +0.08}$ & $^{  +0.17 }_{  -0.00}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  -0.14 }_{  +0.14}$ & $^{  +0.04 }_{  -0.04}$ & $^{  +0.16 }_{  -0.16}$ & $^{  +0.21 }_{  -0.21}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  -0.02 }_{  +0.02}$ & $^{  +0.05 }_{  -0.05}$ & $^{  +0.08 }_{  -0.08}$ & $^{  +0.09 }_{  -0.09}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  -0.01 }_{  +0.01}$ & $^{  +0.02 }_{  -0.02}$ & $^{  +0.05 }_{  -0.05}$ & $^{  +0.06 }_{  -0.06}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  -0.01 }_{  +0.01}$ & $^{  +0.01 }_{  -0.01}$ & $^{  +0.04 }_{  -0.04}$ & $^{  +0.08 }_{  -0.08}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  -1.62 }_{  +1.71}$ & $^{  +2.03 }_{  -2.10}$ & $^{  +2.07 }_{  -1.97}$ & $^{  +1.76 }_{  -1.74}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  -1.22 }_{  +1.10}$ & $^{  +1.53 }_{  -1.22}$ & $^{  +1.54 }_{  -1.31}$ & $^{  +1.45 }_{  -1.47}$ \\ [0.5mm] 
MC generator & $^{  -3.06 }_{  +3.06}$ & $^{  +2.84 }_{  -2.84}$ & $^{  +7.20 }_{  -7.20}$ & $^{  -1.97 }_{  +1.97}$ \\ [0.5mm] 
Fragmentation & $^{  +0.87 }_{  -0.87}$ & $^{  -0.58 }_{  +0.58}$ & $^{  -6.92 }_{  +6.92}$ & $^{  -2.84 }_{  +2.84}$ \\ [0.5mm] 
IFSR & $^{  -4.06 }_{  +4.06}$ & $^{  +0.34 }_{  -0.34}$ & $^{  +4.72 }_{  -4.72}$ & $^{  +8.37 }_{  -8.37}$ \\ [0.5mm] 
PDF & $^{  +0.08 }_{  -0.08}$ & $^{  -0.13 }_{  +0.13}$ & $^{  +0.16 }_{  -0.16}$ & $^{  +1.23 }_{  -1.23}$ \\ [0.5mm] 
MC statistics & $^{  +0.58 }_{  -0.58}$ & $^{  +0.75 }_{  -0.75}$ & $^{  +1.67 }_{  -1.67}$ & $^{  +2.78 }_{  -2.78}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  -0.19 }_{  -0.23}$ & $^{  +0.13 }_{  +0.28}$ & $^{  +0.97 }_{  +0.54}$ & $^{  +1.57 }_{  +0.68}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  -0.19 }_{  +0.40}$ & $^{  +0.13 }_{  -0.39}$ & $^{  +0.97 }_{  -1.47}$ & $^{  +1.57 }_{  -2.18}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  -0.25 }_{  +0.23}$ & $^{  +0.12 }_{  -0.11}$ & $^{  +0.75 }_{  -0.70}$ & $^{  +1.11 }_{  -1.04}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  +0.22 }_{  -0.25}$ & $^{  -0.27 }_{  +0.27}$ & $^{  +0.20 }_{  -0.19}$ & $^{  +0.63 }_{  -0.66}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  +0.03 }_{  -0.32}$ & $^{  -0.01 }_{  +0.24}$ & $^{  +0.34 }_{  +0.59}$ & $^{  +0.68 }_{  +0.73}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  +0.03 }_{  +0.31}$ & $^{  -0.01 }_{  -0.25}$ & $^{  +0.34 }_{  -1.03}$ & $^{  +0.68 }_{  -1.60}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  +0.02 }_{  +0.02}$ & $^{  -0.07 }_{  -0.08}$ & $^{  +0.75 }_{  -1.13}$ & $^{  +1.44 }_{  -1.96}$ \\ [0.5mm] 
Multijet normalization & $^{  -0.11 }_{  +0.11}$ & $^{  +0.32 }_{  -0.33}$ & $^{  +0.28 }_{  -0.28}$ & $^{  +0.14 }_{  -0.13}$ \\ [0.5mm] 
Multijet shape & $^{  +0.03 }_{  +0.04}$ & $^{  -0.13 }_{  -0.07}$ & $^{  +0.18 }_{  -0.34}$ & $^{  +0.43 }_{  -0.45}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  -0.06 }_{  +0.06}$ & $^{  +0.18 }_{  -0.18}$ & $^{  +0.55 }_{  -0.56}$ & $^{  +0.70 }_{  -0.71}$ \\ [0.5mm] 
Dilepton background normalization & $^{  -0.19 }_{  +0.18}$ & $^{  +0.26 }_{  -0.25}$ & $^{  +0.51 }_{  -0.49}$ & $^{  +0.65 }_{  -0.62}$ \\ [0.5mm] 
\hline
Channels BLUE weights  & (0.25 ,0.75) & (0.83 ,0.17) & (0.44 ,0.56) & (0.35 ,0.65) \\ [2mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemPt_Norm_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptttbar}$ Uncertainties [\%] $/$ Bins [GeV] &    [0,  40] &    [40, 170] &    [170, 340] &    [340,1000] \\ 
\hline
\hline
Jet energy scale & $\pm    1.7$ & $^{+    2.0 }_{-    1.7}$ & $^{+    4.7 }_{-    4.5}$ & $\pm    6.1$ \\ [1mm] 
Jet energy resolution & $\pm    3.2$ & $\pm    3.7$ & $\pm    6.9$ & $\pm    7.8$ \\ [1mm] 
Jet reconstruction efficiency & ${\rm --}$ & $\pm    0.2$ & ${\rm --}$ & $\pm    0.2$ \\ [1mm] 
$b$-quark tagging efficiency & $^{\rm --}_{-\rm --}$ & $^{\rm --}_{-\rm --}$ & $^{+    0.4 }_{-    0.2}$ & $^{+    1.0 }_{-    0.2}$ \\ [1mm] 
$c$-quark tagging efficiency & ${\rm --}$ & $\pm    0.2$ & $\pm    0.3$ & $^{+    0.4 }_{-    0.3}$ \\ [1mm] 
Light-jet tagging efficiency & ${\rm --}$ & ${\rm --}$ & $\pm    0.1$ & $\pm    0.2$ \\ [1mm] 
Lepton selection and scaling & $\pm    0.2$ & $^{+    0.4 }_{-    0.3}$ & $^{+    0.5 }_{-    0.4}$ & $^{+    0.9 }_{-    0.7}$ \\ [1mm] 
\Etmiss{} cell-out & $^{+    1.6 }_{-    1.7}$ & $^{+    2.0 }_{-    2.1}$ & $^{+    2.1 }_{-    2.0}$ & $^{+    1.8 }_{-    1.7}$ \\ [1mm] 
\Etmiss{} pile-up & $^{+    1.2 }_{-    1.1}$ & $^{+    1.5 }_{-    1.2}$ & $^{+    1.5 }_{-    1.3}$ & $^{+    1.4 }_{-    1.5}$ \\ [1mm] 
MC generator & $\pm    3.1$ & $\pm    2.8$ & $\pm    7.2$ & $\pm    2.0$ \\ [1mm] 
Fragmentation & $\pm    0.9$ & $\pm    0.6$ & $\pm    6.9$ & $\pm    2.8$ \\ [1mm] 
IFSR & $\pm    4.1$ & $\pm    0.3$ & $\pm    4.7$ & $\pm    8.4$ \\ [1mm] 
PDF & ${\rm --}$ & $\pm    0.1$ & $\pm    0.2$ & $\pm    1.2$ \\ [1mm] 
MC statistics & $\pm    0.6$ & $\pm    0.7$ & $\pm    1.7$ & $\pm    2.8$ \\ [1mm] 
\Wboson+jets & $^{+    0.4 }_{-    0.7}$ & $^{+    0.3 }_{-    0.7}$ & $^{+    1.8 }_{-    2.4}$ & $^{+    3.1 }_{-    3.7}$ \\ [1mm] 
Other backgrounds & $\pm    0.2$ & $\pm    0.5$ & $^{+    0.8 }_{-    0.9}$ & $\pm    1.1$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$1.3 & $\pm$1.8 & $\pm$4.2 & $\pm$7.8 \\ [2mm] 
 Total systematic uncertainty  & $\pm    6.7$ & $^{+    5.8 }_{-    5.7}$ & $\pm   14.3$ & $^{+   14.4 }_{-   14.5}$ \\ [2mm] 
\hline
%%%Channels BLUE weights  & (0.25 ,0.75) & (0.83 ,0.17) & (0.44 ,0.56) & (0.35 ,0.65) \\ [2mm] 
\hline
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemRapidity_NormFinal.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dyttbar}$ Uncertainties [\%] &     -2.5 -- -1.0 &     -1.0 -- -0.5 &     -0.5 --  0.0 &     0.0 --  0.5 &     0.5 --  1.0 &     1.0 --  2.5 \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  +0.11 }_{  -0.01}$ & $^{  -0.02 }_{  +0.04}$ & $^{  +0.16 }_{  -0.11}$ & $^{  -0.08 }_{  -0.03}$ & $^{  -0.22 }_{  +0.03}$ & $^{  +0.05 }_{  +0.17}$ \\ [0.5mm] 
Close-by jets (JES) & $^{  +0.87 }_{  -0.50}$ & $^{  -0.03 }_{  -0.24}$ & $^{  -0.43 }_{  +0.19}$ & $^{  -0.33 }_{  +0.22}$ & $^{  +0.03 }_{  +0.09}$ & $^{  +0.51 }_{  -0.06}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  +0.38 }_{  -0.50}$ & $^{  +0.10 }_{  -0.08}$ & $^{  -0.18 }_{  +0.09}$ & $^{  -0.21 }_{  +0.21}$ & $^{  -0.08 }_{  +0.10}$ & $^{  +0.30 }_{  -0.09}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  +0.02 }_{  +0.03}$ & $^{  -0.01 }_{  -0.01}$ & $^{  +0.01 }_{  -0.02}$ & $^{  +0.02 }_{  +0.02}$ & $^{  -0.04 }_{  +0.06}$ & $^{  -0.01 }_{  -0.09}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  +0.12 }_{  -0.06}$ & $^{  -0.00 }_{  +0.02}$ & $^{  -0.04 }_{  +0.01}$ & $^{  +0.01 }_{  +0.04}$ & $^{  -0.07 }_{  +0.00}$ & $^{  +0.04 }_{  -0.05}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  +0.17 }_{  -0.11}$ & $^{  +0.02 }_{  -0.01}$ & $^{  -0.06 }_{  -0.02}$ & $^{  -0.03 }_{  +0.08}$ & $^{  -0.07 }_{  +0.03}$ & $^{  +0.06 }_{  -0.03}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  +0.14 }_{  -0.18}$ & $^{  +0.06 }_{  -0.07}$ & $^{  -0.05 }_{  -0.12}$ & $^{  -0.12 }_{  +0.28}$ & $^{  -0.08 }_{  -0.00}$ & $^{  +0.20 }_{  -0.01}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  +0.02 }_{  -0.11}$ & $^{  +0.02 }_{  -0.01}$ & $^{  +0.02 }_{  -0.06}$ & $^{  +0.01 }_{  +0.06}$ & $^{  -0.02 }_{  +0.03}$ & $^{  -0.07 }_{  +0.06}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  -0.12 }_{  +0.03}$ & $^{  -0.03 }_{  +0.09}$ & $^{  -0.11 }_{  -0.01}$ & $^{  +0.09 }_{  +0.00}$ & $^{  +0.09 }_{  -0.03}$ & $^{  +0.08 }_{  -0.08}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  +0.08 }_{  +0.03}$ & $^{  -0.05 }_{  -0.05}$ & $^{  +0.01 }_{  +0.05}$ & $^{  +0.07 }_{  +0.04}$ & $^{  -0.07 }_{  -0.04}$ & $^{  -0.05 }_{  -0.06}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  +0.14 }_{  -0.08}$ & $^{  +0.13 }_{  -0.07}$ & $^{  -0.01 }_{  -0.05}$ & $^{  -0.10 }_{  +0.10}$ & $^{  -0.17 }_{  +0.10}$ & $^{  +0.12 }_{  -0.05}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  +0.06 }_{  -0.06}$ & $^{  +0.01 }_{  -0.01}$ & $^{  -0.02 }_{  +0.03}$ & $^{  -0.05 }_{  +0.00}$ & $^{  -0.04 }_{  -0.00}$ & $^{  +0.09 }_{  +0.02}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  +0.17 }_{  -0.00}$ & $^{  +0.07 }_{  -0.08}$ & $^{  -0.07 }_{  +0.00}$ & $^{  -0.09 }_{  +0.06}$ & $^{  -0.03 }_{  -0.04}$ & $^{  +0.07 }_{  +0.05}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  +1.71 }_{  -1.35}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.78 }_{  +0.74}$ & $^{  -0.92 }_{  +0.59}$ & $^{  -0.07 }_{  -0.05}$ & $^{  +1.48 }_{  -1.02}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  +0.36 }_{  -0.18}$ & $^{  +0.01 }_{  -0.09}$ & $^{  -0.15 }_{  -0.06}$ & $^{  -0.06 }_{  +0.05}$ & $^{  -0.04 }_{  +0.11}$ & $^{  +0.07 }_{  +0.17}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  +0.12 }_{  -0.03}$ & $^{  +0.11 }_{  -0.12}$ & $^{  -0.09 }_{  -0.01}$ & $^{  -0.04 }_{  +0.08}$ & $^{  -0.05 }_{  +0.00}$ & $^{  +0.03 }_{  +0.06}$ \\ [0.5mm] 
Flavor response (JES) & $^{  +0.08 }_{  -0.11}$ & $^{  +0.13 }_{  -0.14}$ & $^{  -0.07 }_{  +0.14}$ & $^{  -0.11 }_{  +0.15}$ & $^{  -0.05 }_{  -0.06}$ & $^{  +0.15 }_{  -0.14}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  +0.24 }_{  -0.05}$ & $^{  +0.02 }_{  -0.19}$ & $^{  -0.08 }_{  +0.05}$ & $^{  -0.18 }_{  +0.12}$ & $^{  -0.05 }_{  -0.04}$ & $^{  +0.27 }_{  +0.03}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  +0.07 }_{  +0.00}$ & $^{  -0.03 }_{  +0.16}$ & $^{  -0.16 }_{  -0.01}$ & $^{  -0.01 }_{  -0.12}$ & $^{  +0.07 }_{  +0.00}$ & $^{  +0.17 }_{  +0.02}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  +0.29 }_{  -0.28}$ & $^{  -0.05 }_{  +0.04}$ & $^{  -0.12 }_{  +0.12}$ & $^{  +0.02 }_{  +0.10}$ & $^{  -0.06 }_{  +0.03}$ & $^{  +0.05 }_{  -0.22}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  +0.01 }_{  +0.01}$ & $^{  -0.02 }_{  -0.02}$ & $^{  -0.01 }_{  -0.01}$ & $^{  -0.00 }_{  +0.00}$ & $^{  +0.01 }_{  +0.01}$ & $^{  +0.03 }_{  +0.03}$ \\ [0.5mm] 
JES uncertainty in background & $^{  +0.38 }_{  -1.51}$ & $^{  +0.13 }_{  +0.12}$ & $^{  -0.17 }_{  +0.42}$ & $^{  -0.33 }_{  +0.23}$ & $^{  +0.08 }_{  +0.21}$ & $^{  +0.25 }_{  -0.18}$ \\ [0.5mm] 
Jet energy resolution & $^{  -1.21 }_{  +1.22}$ & $^{  -0.36 }_{  +0.36}$ & $^{  -0.44 }_{  +0.44}$ & $^{  +0.76 }_{  -0.77}$ & $^{  +0.80 }_{  -0.80}$ & $^{  -0.01 }_{  +0.01}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  -0.04 }_{  +0.04}$ & $^{  -0.02 }_{  +0.02}$ & $^{  +0.00 }_{  -0.00}$ & $^{  +0.04 }_{  -0.04}$ & $^{  -0.00 }_{  +0.00}$ & $^{  -0.02 }_{  +0.02}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  +0.23 }_{  -0.26}$ & $^{  +0.14 }_{  -0.13}$ & $^{  +0.11 }_{  -0.10}$ & $^{  -0.08 }_{  +0.09}$ & $^{  -0.16 }_{  +0.17}$ & $^{  -0.24 }_{  +0.22}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  +0.12 }_{  -0.13}$ & $^{  +0.04 }_{  -0.05}$ & $^{  -0.08 }_{  +0.07}$ & $^{  -0.01 }_{  +0.01}$ & $^{  +0.01 }_{  -0.00}$ & $^{  -0.03 }_{  +0.04}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  +0.13 }_{  -0.12}$ & $^{  +0.03 }_{  -0.02}$ & $^{  -0.00 }_{  +0.00}$ & $^{  -0.04 }_{  +0.03}$ & $^{  -0.04 }_{  +0.04}$ & $^{  -0.02 }_{  +0.03}$ \\ [0.5mm] 
$e$ energy resolution & $^{  -0.34 }_{  -0.08}$ & $^{  -0.04 }_{  +0.01}$ & $^{  +0.07 }_{  +0.00}$ & $^{  +0.06 }_{  -0.01}$ & $^{  +0.09 }_{  -0.00}$ & $^{  +0.03 }_{  +0.08}$ \\ [0.5mm] 
$e$ energy scale & $^{  +0.31 }_{  -0.40}$ & $^{  +0.15 }_{  -0.12}$ & $^{  -0.09 }_{  +0.09}$ & $^{  -0.10 }_{  +0.14}$ & $^{  -0.08 }_{  +0.06}$ & $^{  -0.04 }_{  +0.05}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  +0.07 }_{  -0.04}$ & $^{  -0.09 }_{  -0.16}$ & $^{  -0.08 }_{  -0.03}$ & $^{  +0.15 }_{  +0.14}$ & $^{  +0.00 }_{  +0.04}$ & $^{  -0.08 }_{  +0.01}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  +0.13 }_{  +0.08}$ & $^{  -0.00 }_{  +0.05}$ & $^{  -0.10 }_{  -0.12}$ & $^{  -0.00 }_{  -0.08}$ & $^{  +0.04 }_{  +0.06}$ & $^{  +0.02 }_{  +0.14}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  +0.05 }_{  -0.05}$ & $^{  +0.03 }_{  -0.03}$ & $^{  +0.08 }_{  -0.08}$ & $^{  -0.02 }_{  +0.02}$ & $^{  +0.00 }_{  -0.00}$ & $^{  -0.18 }_{  +0.18}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  +1.02 }_{  -0.99}$ & $^{  +0.19 }_{  -0.19}$ & $^{  -0.36 }_{  +0.35}$ & $^{  -0.60 }_{  +0.58}$ & $^{  -0.13 }_{  +0.12}$ & $^{  +0.65 }_{  -0.62}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  +0.28 }_{  -0.28}$ & $^{  +0.11 }_{  -0.11}$ & $^{  -0.10 }_{  +0.10}$ & $^{  -0.21 }_{  +0.21}$ & $^{  -0.01 }_{  +0.01}$ & $^{  +0.15 }_{  -0.15}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  -0.52 }_{  +0.51}$ & $^{  -0.14 }_{  +0.14}$ & $^{  +0.22 }_{  -0.22}$ & $^{  +0.35 }_{  -0.35}$ & $^{  +0.02 }_{  -0.02}$ & $^{  -0.36 }_{  +0.35}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  -0.38 }_{  -0.27}$ & $^{  -0.13 }_{  +0.03}$ & $^{  +0.19 }_{  -0.01}$ & $^{  +0.18 }_{  -0.18}$ & $^{  -0.06 }_{  +0.14}$ & $^{  -0.07 }_{  +0.35}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  -0.35 }_{  -0.22}$ & $^{  +0.01 }_{  +0.10}$ & $^{  +0.12 }_{  +0.21}$ & $^{  +0.18 }_{  -0.14}$ & $^{  -0.08 }_{  -0.06}$ & $^{  -0.10 }_{  +0.03}$ \\ [0.5mm] 
MC generator & $^{  +2.70 }_{  -3.34}$ & $^{  -1.43 }_{  +1.77}$ & $^{  -1.48 }_{  +1.84}$ & $^{  -1.53 }_{  +1.90}$ & $^{  -0.12 }_{  +0.14}$ & $^{  +4.69 }_{  -5.80}$ \\ [0.5mm] 
Fragmentation & $^{  +2.23 }_{  -2.14}$ & $^{  -1.94 }_{  +1.86}$ & $^{  -1.42 }_{  +1.37}$ & $^{  -0.58 }_{  +0.56}$ & $^{  +0.78 }_{  -0.75}$ & $^{  +2.88 }_{  -2.77}$ \\ [0.5mm] 
IFSR & $^{  -2.41 }_{  +2.36}$ & $^{  -1.52 }_{  +1.48}$ & $^{  -0.08 }_{  +0.08}$ & $^{  +1.06 }_{  -1.04}$ & $^{  +1.06 }_{  -1.04}$ & $^{  +1.06 }_{  -1.04}$ \\ [0.5mm] 
PDF & $^{  +1.37 }_{  -1.40}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.74 }_{  +0.75}$ & $^{  -0.75 }_{  +0.76}$ & $^{  -0.03 }_{  +0.03}$ & $^{  +1.39 }_{  -1.41}$ \\ [0.5mm] 
MC statistics & $^{  +0.64 }_{  -0.64}$ & $^{  +0.34 }_{  -0.34}$ & $^{  +0.37 }_{  -0.37}$ & $^{  +0.35 }_{  -0.35}$ & $^{  +0.36 }_{  -0.36}$ & $^{  +0.66 }_{  -0.66}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  +0.17 }_{  -0.13}$ & $^{  +0.00 }_{  +0.00}$ & $^{  -0.11 }_{  +0.09}$ & $^{  -0.15 }_{  +0.06}$ & $^{  +0.04 }_{  -0.02}$ & $^{  +0.23 }_{  -0.11}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  +0.17 }_{  -0.04}$ & $^{  +0.00 }_{  -0.01}$ & $^{  -0.11 }_{  +0.02}$ & $^{  -0.15 }_{  +0.09}$ & $^{  +0.04 }_{  -0.02}$ & $^{  +0.23 }_{  -0.12}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  +0.31 }_{  -0.30}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.40 }_{  +0.38}$ & $^{  -0.40 }_{  +0.38}$ & $^{  +0.21 }_{  -0.20}$ & $^{  +0.87 }_{  -0.83}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  +0.37 }_{  -0.25}$ & $^{  +0.04 }_{  -0.01}$ & $^{  -0.07 }_{  +0.02}$ & $^{  -0.11 }_{  +0.05}$ & $^{  -0.07 }_{  +0.06}$ & $^{  +0.02 }_{  +0.05}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  -0.13 }_{  +0.07}$ & $^{  -0.02 }_{  +0.03}$ & $^{  +0.13 }_{  -0.09}$ & $^{  +0.17 }_{  -0.07}$ & $^{  -0.06 }_{  +0.03}$ & $^{  -0.31 }_{  +0.15}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  -0.13 }_{  +0.08}$ & $^{  -0.02 }_{  -0.01}$ & $^{  +0.13 }_{  -0.06}$ & $^{  +0.17 }_{  -0.13}$ & $^{  -0.06 }_{  +0.04}$ & $^{  -0.31 }_{  +0.20}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  +0.26 }_{  -0.33}$ & $^{  +0.01 }_{  -0.01}$ & $^{  -0.07 }_{  +0.09}$ & $^{  -0.12 }_{  +0.15}$ & $^{  -0.00 }_{  +0.01}$ & $^{  +0.08 }_{  -0.11}$ \\ [0.5mm] 
Multijet normalization & $^{  +1.97 }_{  -1.96}$ & $^{  +0.13 }_{  -0.13}$ & $^{  -0.44 }_{  +0.44}$ & $^{  -0.65 }_{  +0.65}$ & $^{  -0.29 }_{  +0.29}$ & $^{  +0.31 }_{  -0.32}$ \\ [0.5mm] 
Multijet shape & $^{  +0.29 }_{  -0.90}$ & $^{  -0.07 }_{  +0.06}$ & $^{  -0.14 }_{  +0.16}$ & $^{  -0.14 }_{  +0.19}$ & $^{  -0.07 }_{  +0.12}$ & $^{  +0.41 }_{  -0.02}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  +0.61 }_{  -0.62}$ & $^{  +0.01 }_{  -0.02}$ & $^{  -0.17 }_{  +0.17}$ & $^{  -0.26 }_{  +0.26}$ & $^{  -0.11 }_{  +0.11}$ & $^{  +0.30 }_{  -0.30}$ \\ [0.5mm] 
Dilepton background normalization & $^{  +0.08 }_{  -0.08}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.00 }_{  +0.00}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.04 }_{  +0.04}$ \\ [0.5mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_SystemRapidity_NormFinal_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dyttbar}$ Uncertainties [\%] &     -2.5 -- -1.0 &     -1.0 -- -0.5 &     -0.5 --  0.0 &     0.0 --  0.5 &     0.5 --  1.0 &     1.0 --  2.5 \\ 
\hline
\hline
Jet energy scale & $^{+    2.1 }_{-    2.2}$ & $^{+    0.3 }_{-    0.5}$ & $^{+    1.0 }_{-    0.9}$ & $^{+    1.1 }_{-    0.8}$ & $^{+    0.4 }_{-    0.3}$ & $^{+    1.7 }_{-    1.1}$ \\ [1mm] 
Jet energy resolution & $\pm    1.2$ & $\pm    0.4$ & $\pm    0.4$ & $\pm    0.8$ & $\pm    0.8$ & ${\rm --}$ \\ [1mm] 
Jet reconstruction efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
$b$-quark tagging efficiency & $^{+    0.2 }_{-    0.3}$ & $\pm    0.1$ & $\pm    0.1$ & ${\rm --}$ & $\pm    0.2$ & $\pm    0.2$ \\ [1mm] 
$c$-quark tagging efficiency & $\pm    0.1$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Light-jet tagging efficiency & $\pm    0.1$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Lepton selection and momentum scale & $^{+    1.3 }_{-    1.2}$ & $\pm    0.3$ & $\pm    0.5$ & $^{+    0.8 }_{-    0.7}$ & $\pm    0.2$ & $\pm    0.8$ \\ [1mm] 
\Etmiss{} cell-out & $^{\rm --}_{-    0.4}$ & $^{\rm --}_{-    0.1}$ & $^{+    0.2 }_{\rm --}$ & $\pm    0.2$ & $\pm    0.1$ & $^{+    0.3 }_{\rm --}$ \\ [1mm] 
\Etmiss{} pile-up & $^{\rm --}_{-    0.3}$ & ${\rm --}$ & $^{+    0.2 }_{\rm --}$ & $^{+    0.2 }_{-    0.1}$ & ${\rm --}$ & $^{\rm --}_{-    0.1}$ \\ [1mm] 
MC generator & $^{+    2.7 }_{-    3.3}$ & $^{+    1.8 }_{-    1.4}$ & $^{+    1.8 }_{-    1.5}$ & $^{+    1.9 }_{-    1.5}$ & $\pm    0.1$ & $^{+    4.7 }_{-    5.8}$ \\ [1mm] 
Fragmentation & $^{+    2.2 }_{-    2.1}$ & $\pm    1.9$ & $\pm    1.4$ & $\pm    0.6$ & $\pm    0.8$ & $^{+    2.9 }_{-    2.8}$ \\ [1mm] 
IFSR & $\pm    2.4$ & $\pm    1.5$ & ${\rm --}$ & $^{+    1.1 }_{-    1.0}$ & $^{+    1.1 }_{-    1.0}$ & $^{+    1.1 }_{-    1.0}$ \\ [1mm] 
PDF & $\pm    1.4$ & ${\rm --}$ & $\pm    0.7$ & $^{+    0.8 }_{-    0.7}$ & ${\rm --}$ & $\pm    1.4$ \\ [1mm] 
MC statistics & $\pm    0.6$ & $\pm    0.3$ & $\pm    0.4$ & $\pm    0.3$ & $\pm    0.4$ & $\pm    0.7$ \\ [1mm] 
\Wboson+jets & $^{+    0.6 }_{-    0.5}$ & ${\rm --}$ & $^{+    0.5 }_{-    0.4}$ & $\pm    0.5$ & $^{+    0.3 }_{-    0.2}$ & $^{+    1.0 }_{-    0.9}$ \\ [1mm] 
Other backgrounds & $^{+    2.1 }_{-    2.2}$ & $\pm    0.1$ & $\pm    0.5$ & $\pm    0.7$ & $\pm    0.3$ & $^{+    0.6 }_{-    0.4}$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$2.3 & $\pm$1.2 & $\pm$1.3 & $\pm$1.2 & $\pm$1.2 & $\pm$2.7 \\ [2mm] 
 Total systematic uncertainty  & $^{+    5.7 }_{-    6.1}$ & $\pm    3.0$ & $^{+    2.8 }_{-    2.6}$ & $^{+    3.0 }_{-    2.7}$ & $\pm    1.7$ & $^{+    6.2 }_{-    6.9}$ \\ [2mm] 
\hline
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_Top1_lhood_NormFinal.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptt}$ Uncertainties [\%] $/$ Bins [GeV] &     0--50 &     50--100 &     100--150 &     150--200 &     200--250 &     250--350 &     350--800 \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  -1.80 }_{  +1.54}$ & $^{  -0.43 }_{  +0.37}$ & $^{  +0.99 }_{  -0.92}$ & $^{  +1.07 }_{  -0.64}$ & $^{  +0.72 }_{  -0.65}$ & $^{  +0.36 }_{  -0.70}$ & $^{  +0.02 }_{  -0.83}$ \\ [0.5mm] 
Close-by jets (JES) & $^{  -1.32 }_{  +1.40}$ & $^{  -0.52 }_{  +0.66}$ & $^{  +0.31 }_{  -0.67}$ & $^{  +0.95 }_{  -1.01}$ & $^{  +1.66 }_{  -1.09}$ & $^{  +2.18 }_{  -1.98}$ & $^{  +2.71 }_{  -2.95}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  -1.84 }_{  +1.32}$ & $^{  -0.61 }_{  +0.51}$ & $^{  +0.56 }_{  -0.51}$ & $^{  +1.12 }_{  -0.66}$ & $^{  +2.11 }_{  -1.34}$ & $^{  +2.46 }_{  -2.31}$ & $^{  +2.59 }_{  -2.71}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  -0.28 }_{  +0.06}$ & $^{  -0.06 }_{  +0.01}$ & $^{  +0.12 }_{  -0.09}$ & $^{  +0.15 }_{  +0.11}$ & $^{  +0.27 }_{  -0.01}$ & $^{  +0.09 }_{  -0.11}$ & $^{  -0.04 }_{  -0.04}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  -0.25 }_{  -0.10}$ & $^{  +0.05 }_{  -0.00}$ & $^{  -0.02 }_{  -0.08}$ & $^{  +0.06 }_{  +0.23}$ & $^{  +0.13 }_{  +0.26}$ & $^{  +0.31 }_{  -0.16}$ & $^{  +0.63 }_{  -0.49}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  -0.18 }_{  -0.08}$ & $^{  -0.08 }_{  +0.12}$ & $^{  +0.20 }_{  -0.25}$ & $^{  +0.15 }_{  +0.18}$ & $^{  -0.10 }_{  +0.21}$ & $^{  -0.16 }_{  +0.02}$ & $^{  -0.41 }_{  +0.05}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  -0.53 }_{  +0.75}$ & $^{  -0.07 }_{  +0.26}$ & $^{  +0.04 }_{  -0.57}$ & $^{  +0.39 }_{  -0.45}$ & $^{  +0.81 }_{  -0.04}$ & $^{  +0.23 }_{  -0.13}$ & $^{  -0.20 }_{  -0.05}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  -0.61 }_{  +0.41}$ & $^{  -0.16 }_{  +0.28}$ & $^{  -0.00 }_{  -0.19}$ & $^{  +0.51 }_{  -0.42}$ & $^{  +0.80 }_{  -0.48}$ & $^{  +0.98 }_{  -0.70}$ & $^{  +1.25 }_{  -0.78}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  +0.65 }_{  -0.83}$ & $^{  +0.30 }_{  -0.24}$ & $^{  -0.35 }_{  +0.19}$ & $^{  -0.41 }_{  +0.65}$ & $^{  -0.48 }_{  +0.86}$ & $^{  -0.91 }_{  +0.89}$ & $^{  -1.16 }_{  +0.88}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  -0.31 }_{  +0.02}$ & $^{  -0.03 }_{  +0.08}$ & $^{  +0.02 }_{  -0.13}$ & $^{  +0.25 }_{  +0.09}$ & $^{  +0.34 }_{  +0.05}$ & $^{  +0.15 }_{  -0.23}$ & $^{  +0.14 }_{  -0.41}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  +0.05 }_{  -0.17}$ & $^{  +0.06 }_{  +0.04}$ & $^{  +0.08 }_{  -0.29}$ & $^{  -0.17 }_{  +0.15}$ & $^{  -0.18 }_{  +0.76}$ & $^{  -0.37 }_{  +0.61}$ & $^{  -0.48 }_{  +0.71}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  -0.24 }_{  +0.02}$ & $^{  -0.03 }_{  +0.06}$ & $^{  -0.01 }_{  -0.09}$ & $^{  +0.25 }_{  +0.08}$ & $^{  +0.27 }_{  +0.04}$ & $^{  +0.12 }_{  -0.26}$ & $^{  +0.17 }_{  -0.29}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  -0.43 }_{  +0.31}$ & $^{  -0.13 }_{  +0.29}$ & $^{  +0.08 }_{  -0.26}$ & $^{  +0.27 }_{  -0.32}$ & $^{  +0.49 }_{  -0.32}$ & $^{  +0.73 }_{  -0.55}$ & $^{  +1.11 }_{  -0.54}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  -1.47 }_{  +1.29}$ & $^{  -0.68 }_{  +0.55}$ & $^{  +0.49 }_{  -0.88}$ & $^{  +1.59 }_{  -0.74}$ & $^{  +1.60 }_{  -0.40}$ & $^{  +1.17 }_{  -1.21}$ & $^{  +0.88 }_{  -1.63}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  -0.42 }_{  -0.02}$ & $^{  -0.06 }_{  +0.10}$ & $^{  +0.07 }_{  -0.16}$ & $^{  +0.31 }_{  +0.02}$ & $^{  +0.43 }_{  +0.15}$ & $^{  +0.21 }_{  -0.07}$ & $^{  +0.13 }_{  +0.12}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  -0.32 }_{  +0.14}$ & $^{  -0.00 }_{  +0.27}$ & $^{  +0.03 }_{  -0.28}$ & $^{  +0.03 }_{  -0.12}$ & $^{  +0.33 }_{  -0.02}$ & $^{  +0.57 }_{  -0.55}$ & $^{  +0.77 }_{  -1.10}$ \\ [0.5mm] 
Flavor response (JES) & $^{  +0.15 }_{  -0.03}$ & $^{  +0.09 }_{  +0.16}$ & $^{  -0.29 }_{  -0.30}$ & $^{  -0.18 }_{  +0.05}$ & $^{  +0.38 }_{  +0.42}$ & $^{  +0.44 }_{  +0.03}$ & $^{  +0.62 }_{  -0.09}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  +0.08 }_{  +0.13}$ & $^{  +0.01 }_{  +0.09}$ & $^{  -0.05 }_{  -0.16}$ & $^{  -0.07 }_{  -0.02}$ & $^{  +0.07 }_{  +0.07}$ & $^{  +0.09 }_{  -0.34}$ & $^{  -0.13 }_{  -0.30}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  +0.08 }_{  -0.38}$ & $^{  +0.08 }_{  +0.01}$ & $^{  -0.03 }_{  -0.03}$ & $^{  -0.05 }_{  +0.18}$ & $^{  -0.09 }_{  +0.60}$ & $^{  -0.40 }_{  +0.34}$ & $^{  -0.64 }_{  +0.12}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  -0.25 }_{  +0.03}$ & $^{  -0.03 }_{  -0.05}$ & $^{  +0.08 }_{  -0.00}$ & $^{  +0.02 }_{  +0.21}$ & $^{  +0.28 }_{  -0.03}$ & $^{  +0.27 }_{  -0.31}$ & $^{  +0.26 }_{  -0.40}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  -0.06 }_{  -0.06}$ & $^{  +0.01 }_{  +0.01}$ & $^{  +0.03 }_{  +0.03}$ & $^{  +0.00 }_{  -0.01}$ & $^{  +0.01 }_{  +0.00}$ & $^{  +0.00 }_{  +0.01}$ & $^{  +0.01 }_{  +0.01}$ \\ [0.5mm] 
JES uncertainty in background & $^{  -0.58 }_{  +0.02}$ & $^{  -0.26 }_{  +0.06}$ & $^{  +0.53 }_{  -0.21}$ & $^{  +0.66 }_{  -0.08}$ & $^{  -0.51 }_{  +0.34}$ & $^{  -0.16 }_{  +0.53}$ & $^{  -0.37 }_{  +0.41}$ \\ [0.5mm] 
Jet energy resolution & $^{  +1.56 }_{  -1.56}$ & $^{  +0.31 }_{  -0.31}$ & $^{  -1.24 }_{  +1.24}$ & $^{  -0.13 }_{  +0.13}$ & $^{  +0.07 }_{  -0.07}$ & $^{  -0.63 }_{  +0.64}$ & $^{  -2.00 }_{  +2.00}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  -0.02 }_{  +0.02}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.07 }_{  +0.07}$ & $^{  +0.08 }_{  -0.08}$ & $^{  +0.06 }_{  -0.06}$ & $^{  -0.04 }_{  +0.04}$ & $^{  -0.17 }_{  +0.17}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  -1.46 }_{  +1.21}$ & $^{  -0.90 }_{  +0.71}$ & $^{  +0.07 }_{  -0.14}$ & $^{  +1.56 }_{  -1.27}$ & $^{  +2.97 }_{  -2.32}$ & $^{  +3.60 }_{  -2.55}$ & $^{  +3.97 }_{  -2.57}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  -0.06 }_{  +0.04}$ & $^{  -0.04 }_{  +0.03}$ & $^{  +0.11 }_{  -0.09}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.09 }_{  +0.09}$ & $^{  -0.13 }_{  +0.13}$ & $^{  -0.19 }_{  +0.20}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  +0.26 }_{  -0.26}$ & $^{  +0.11 }_{  -0.10}$ & $^{  -0.19 }_{  +0.20}$ & $^{  -0.16 }_{  +0.15}$ & $^{  -0.16 }_{  +0.14}$ & $^{  -0.03 }_{  +0.01}$ & $^{  +0.09 }_{  -0.09}$ \\ [0.5mm] 
$e$ energy resolution & $^{  -0.08 }_{  -0.16}$ & $^{  +0.03 }_{  +0.06}$ & $^{  -0.00 }_{  +0.03}$ & $^{  +0.06 }_{  -0.05}$ & $^{  +0.09 }_{  +0.03}$ & $^{  -0.17 }_{  +0.17}$ & $^{  -0.32 }_{  +0.13}$ \\ [0.5mm] 
$e$ energy scale & $^{  +0.15 }_{  -0.38}$ & $^{  +0.14 }_{  -0.08}$ & $^{  -0.21 }_{  +0.21}$ & $^{  -0.13 }_{  +0.27}$ & $^{  -0.01 }_{  +0.07}$ & $^{  -0.07 }_{  -0.08}$ & $^{  -0.10 }_{  +0.01}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  +0.27 }_{  +0.15}$ & $^{  +0.00 }_{  -0.08}$ & $^{  -0.37 }_{  -0.26}$ & $^{  +0.18 }_{  +0.32}$ & $^{  +0.38 }_{  +0.33}$ & $^{  +0.06 }_{  +0.14}$ & $^{  -0.12 }_{  +0.21}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  +0.24 }_{  +0.18}$ & $^{  -0.02 }_{  -0.00}$ & $^{  -0.29 }_{  -0.26}$ & $^{  +0.23 }_{  +0.25}$ & $^{  +0.23 }_{  +0.21}$ & $^{  -0.05 }_{  -0.13}$ & $^{  -0.04 }_{  -0.44}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  +0.03 }_{  -0.03}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.21 }_{  +0.21}$ & $^{  +0.26 }_{  -0.26}$ & $^{  +0.46 }_{  -0.46}$ & $^{  +0.30 }_{  -0.30}$ & $^{  +0.24 }_{  -0.24}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  +0.91 }_{  -0.88}$ & $^{  +0.59 }_{  -0.57}$ & $^{  -0.97 }_{  +0.93}$ & $^{  -0.89 }_{  +0.85}$ & $^{  -0.22 }_{  +0.21}$ & $^{  +0.65 }_{  -0.62}$ & $^{  +0.50 }_{  -0.48}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  +0.34 }_{  -0.33}$ & $^{  +0.22 }_{  -0.21}$ & $^{  -0.37 }_{  +0.36}$ & $^{  -0.33 }_{  +0.32}$ & $^{  -0.07 }_{  +0.07}$ & $^{  +0.27 }_{  -0.26}$ & $^{  +0.23 }_{  -0.22}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  -0.39 }_{  +0.39}$ & $^{  -0.27 }_{  +0.27}$ & $^{  +0.45 }_{  -0.45}$ & $^{  +0.40 }_{  -0.40}$ & $^{  +0.06 }_{  -0.06}$ & $^{  -0.38 }_{  +0.38}$ & $^{  -0.32 }_{  +0.32}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  -0.64 }_{  +0.04}$ & $^{  -0.07 }_{  +0.06}$ & $^{  +0.29 }_{  -0.60}$ & $^{  +0.24 }_{  +0.62}$ & $^{  +0.52 }_{  +0.54}$ & $^{  +0.07 }_{  +0.32}$ & $^{  -0.58 }_{  +0.26}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  -0.50 }_{  +0.17}$ & $^{  -0.11 }_{  -0.13}$ & $^{  +0.08 }_{  -0.23}$ & $^{  +0.53 }_{  +0.47}$ & $^{  +0.62 }_{  +0.17}$ & $^{  -0.02 }_{  -0.01}$ & $^{  -0.47 }_{  +0.11}$ \\ [0.5mm] 
MC generator & $^{  -2.96 }_{  +3.65}$ & $^{  +0.36 }_{  -0.45}$ & $^{  +0.48 }_{  -0.60}$ & $^{  +1.43 }_{  -1.77}$ & $^{  +1.48 }_{  -1.82}$ & $^{  +0.65 }_{  -0.80}$ & $^{  -4.54 }_{  +5.61}$ \\ [0.5mm] 
Fragmentation & $^{  -1.02 }_{  +0.98}$ & $^{  +0.57 }_{  -0.56}$ & $^{  -1.20 }_{  +1.16}$ & $^{  +1.09 }_{  -1.05}$ & $^{  +1.09 }_{  -1.05}$ & $^{  +0.83 }_{  -0.80}$ & $^{  +6.16 }_{  -5.95}$ \\ [0.5mm] 
IFSR & $^{  +2.73 }_{  -2.62}$ & $^{  +1.07 }_{  -1.02}$ & $^{  -0.78 }_{  +0.74}$ & $^{  -2.03 }_{  +1.95}$ & $^{  -2.97 }_{  +2.84}$ & $^{  -3.92 }_{  +3.75}$ & $^{  -5.98 }_{  +5.73}$ \\ [0.5mm] 
PDF & $^{  +0.42 }_{  -0.44}$ & $^{  +0.33 }_{  -0.34}$ & $^{  -0.18 }_{  +0.19}$ & $^{  -0.51 }_{  +0.52}$ & $^{  -0.61 }_{  +0.63}$ & $^{  -0.75 }_{  +0.77}$ & $^{  -0.73 }_{  +0.76}$ \\ [0.5mm] 
MC statistics & $^{  +0.94 }_{  -0.94}$ & $^{  +0.37 }_{  -0.37}$ & $^{  +0.65 }_{  -0.65}$ & $^{  +0.79 }_{  -0.79}$ & $^{  +0.94 }_{  -0.94}$ & $^{  +1.27 }_{  -1.27}$ & $^{  +2.12 }_{  -2.12}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  +0.33 }_{  -0.32}$ & $^{  +0.02 }_{  -0.05}$ & $^{  -0.12 }_{  +0.07}$ & $^{  -0.15 }_{  +0.15}$ & $^{  -0.18 }_{  +0.30}$ & $^{  -0.08 }_{  +0.32}$ & $^{  -0.08 }_{  +0.39}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  +0.33 }_{  -0.02}$ & $^{  +0.02 }_{  +0.03}$ & $^{  -0.12 }_{  +0.04}$ & $^{  -0.15 }_{  +0.00}$ & $^{  -0.18 }_{  -0.12}$ & $^{  -0.08 }_{  -0.23}$ & $^{  -0.08 }_{  -0.30}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  +0.04 }_{  -0.06}$ & $^{  -0.17 }_{  +0.15}$ & $^{  -0.06 }_{  +0.08}$ & $^{  +0.36 }_{  -0.33}$ & $^{  +0.17 }_{  -0.16}$ & $^{  +0.17 }_{  -0.17}$ & $^{  +0.26 }_{  -0.26}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  +1.01 }_{  -0.99}$ & $^{  +0.28 }_{  -0.25}$ & $^{  -0.36 }_{  +0.28}$ & $^{  -0.77 }_{  +0.76}$ & $^{  -0.80 }_{  +0.86}$ & $^{  -0.59 }_{  +0.70}$ & $^{  -0.76 }_{  +0.87}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  +0.27 }_{  -0.30}$ & $^{  +0.09 }_{  -0.10}$ & $^{  +0.06 }_{  +0.08}$ & $^{  -0.36 }_{  +0.26}$ & $^{  -0.42 }_{  +0.30}$ & $^{  -0.46 }_{  +0.29}$ & $^{  -0.51 }_{  +0.32}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  +0.27 }_{  +0.01}$ & $^{  +0.09 }_{  +0.01}$ & $^{  +0.06 }_{  -0.16}$ & $^{  -0.36 }_{  +0.14}$ & $^{  -0.42 }_{  +0.16}$ & $^{  -0.46 }_{  +0.22}$ & $^{  -0.51 }_{  +0.25}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  +0.74 }_{  -0.87}$ & $^{  +0.20 }_{  -0.26}$ & $^{  -0.25 }_{  +0.31}$ & $^{  -0.56 }_{  +0.69}$ & $^{  -0.60 }_{  +0.70}$ & $^{  -0.51 }_{  +0.53}$ & $^{  -0.50 }_{  +0.52}$ \\ [0.5mm] 
Multijet normalization & $^{  +2.27 }_{  -2.29}$ & $^{  +0.26 }_{  -0.27}$ & $^{  -1.09 }_{  +1.11}$ & $^{  -0.99 }_{  +1.00}$ & $^{  -0.86 }_{  +0.87}$ & $^{  -0.39 }_{  +0.39}$ & $^{  -0.06 }_{  +0.05}$ \\ [0.5mm] 
Multijet shape & $^{  +0.60 }_{  -1.58}$ & $^{  +0.12 }_{  +0.19}$ & $^{  -0.37 }_{  +0.40}$ & $^{  -0.52 }_{  +0.52}$ & $^{  -0.03 }_{  +0.48}$ & $^{  +0.64 }_{  +0.13}$ & $^{  +0.36 }_{  +0.09}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  +0.63 }_{  -0.64}$ & $^{  +0.25 }_{  -0.25}$ & $^{  -0.41 }_{  +0.41}$ & $^{  -0.42 }_{  +0.42}$ & $^{  -0.38 }_{  +0.38}$ & $^{  -0.17 }_{  +0.17}$ & $^{  -0.22 }_{  +0.22}$ \\ [0.5mm] 
Dilepton background normalization & $^{  +0.14 }_{  -0.13}$ & $^{  +0.09 }_{  -0.09}$ & $^{  -0.04 }_{  +0.04}$ & $^{  -0.15 }_{  +0.15}$ & $^{  -0.23 }_{  +0.22}$ & $^{  -0.21 }_{  +0.19}$ & $^{  -0.20 }_{  +0.19}$ \\ [0.5mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_Top1_lhood_NormFinal_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptt}$ Uncertainties [\%] $/$ Bins [GeV] &     0 --   50 &     50 --  100 &     100 --  150 &     150 --  200 &     200 --  250 &     250 --  350 &     350 --  800 \\ 
\hline
\hline
Jet energy scale & $^{+    3.6 }_{-    3.1}$ & $^{+    1.2 }_{-    1.3}$ & $^{+    1.5 }_{-    1.8}$ & $^{+    2.7 }_{-    1.9}$ & $^{+    3.6 }_{-    2.4}$ & $^{+    4.0 }_{-    3.8}$ & $^{+    4.6 }_{-    4.9}$ \\ [1mm] 
Jet energy resolution & $\pm    1.6$ & $\pm    0.3$ & $\pm    1.2$ & $\pm    0.1$ & ${\rm --}$ & $\pm    0.6$ & $\pm    2.0$ \\ [1mm] 
Jet reconstruction efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & $\pm    0.2$ \\ [1mm] 
$b$-quark tagging efficiency & $^{+    1.2 }_{-    1.5}$ & $^{+    0.7 }_{-    0.9}$ & ${\rm --}$ & $^{+    1.6 }_{-    1.3}$ & $^{+    3.0 }_{-    2.3}$ & $^{+    3.6 }_{-    2.6}$ & $^{+    4.0 }_{-    2.6}$ \\ [1mm] 
$c$-quark tagging efficiency & ${\rm --}$ & ${\rm --}$ & $\pm    0.1$ & ${\rm --}$ & ${\rm --}$ & $\pm    0.1$ & $\pm    0.2$ \\ [1mm] 
Light-jet tagging efficiency & $\pm    0.3$ & $\pm    0.1$ & $\pm    0.2$ & $^{+    0.1 }_{-    0.2}$ & $^{+    0.1 }_{-    0.2}$ & ${\rm --}$ & ${\rm --}$ \\ [1mm] 
Lepton selection and momentum scale & $\pm    1.1$ & $\pm    0.7$ & $^{+    1.3 }_{-    1.2}$ & $\pm    1.1$ & $^{+    0.7 }_{-    0.6}$ & $\pm    0.9$ & $\pm    0.8$ \\ [1mm] 
\Etmiss{} cell-out & $^{\rm --}_{-    0.6}$ & ${\rm --}$ & $^{+    0.3 }_{-    0.6}$ & $^{+    0.6 }_{\rm --}$ & $^{+    0.5 }_{\rm --}$ & $^{+    0.3 }_{\rm --}$ & $^{+    0.3 }_{-    0.6}$ \\ [1mm] 
\Etmiss{} pile-up & $^{+    0.2 }_{-    0.5}$ & $^{\rm --}_{-    0.1}$ & $^{\rm --}_{-    0.2}$ & $^{+    0.5 }_{\rm --}$ & $^{+    0.6 }_{\rm --}$ & ${\rm --}$ & $^{+    0.1 }_{-    0.5}$ \\ [1mm] 
MC generator & $^{+    3.7 }_{-    3.0}$ & $^{+    0.4 }_{-    0.5}$ & $^{+    0.5 }_{-    0.6}$ & $^{+    1.4 }_{-    1.8}$ & $^{+    1.5 }_{-    1.8}$ & $^{+    0.6 }_{-    0.8}$ & $^{+    5.6 }_{-    4.5}$ \\ [1mm] 
Fragmentation & $\pm    1.0$ & $\pm    0.6$ & $\pm    1.2$ & $\pm    1.1$ & $\pm    1.1$ & $\pm    0.8$ & $^{+    6.2 }_{-    6.0}$ \\ [1mm] 
IFSR & $^{+    2.7 }_{-    2.6}$ & $^{+    1.1 }_{-    1.0}$ & $^{+    0.7 }_{-    0.8}$ & $^{+    1.9 }_{-    2.0}$ & $^{+    2.8 }_{-    3.0}$ & $^{+    3.8 }_{-    3.9}$ & $^{+    5.7 }_{-    6.0}$ \\ [1mm] 
PDF & $\pm    0.4$ & $\pm    0.3$ & $\pm    0.2$ & $\pm    0.5$ & $\pm    0.6$ & $^{+    0.8 }_{-    0.7}$ & $^{+    0.8 }_{-    0.7}$ \\ [1mm] 
MC statistics & $\pm    0.9$ & $\pm    0.4$ & $\pm    0.6$ & $\pm    0.8$ & $\pm    0.9$ & $\pm    1.3$ & $\pm    2.1$ \\ [1mm] 
\Wboson+jets & $\pm    1.4$ & $\pm    0.4$ & $\pm    0.5$ & $^{+    1.2 }_{-    1.1}$ & $\pm    1.2$ & $\pm    1.0$ & $\pm    1.2$ \\ [1mm] 
Other backgrounds & $^{+    2.4 }_{-    2.9}$ & $\pm    0.4$ & $^{+    1.2 }_{-    1.3}$ & $\pm    1.2$ & $^{+    1.0 }_{-    1.1}$ & $^{+    0.8 }_{-    0.5}$ & $^{+    0.5 }_{-    0.3}$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$2.1 & $\pm$0.9 & $\pm$1.4 & $\pm$1.8 & $\pm$2.2 & $\pm$3.0 & $\pm$5.1 \\ [2mm] 
 Total systematic uncertainty  & $^{+    7.0 }_{-    6.6}$ & $^{+    2.2 }_{-    2.3}$ & $^{+    3.1 }_{-    3.4}$ & $^{+    4.7 }_{-    4.3}$ & $^{+    6.2 }_{-    5.4}$ & $^{+    7.0 }_{-    6.5}$ & $\pm 12$ \\ [2mm] 
\hline
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_Top2_lhood_Norm.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptt}$ Uncertainties [\%] $/$ Bins [GeV] &    [0,  50] &    [50, 100] &    [100, 150] &    [150, 200] &    [200, 250] &    [250, 350] &    [350, 800] \\ 
\hline
\hline
$b$-quark jets (JES)  & $^{  -1.72 }_{  +1.50}$ & $^{  -0.33 }_{  +0.44}$ & $^{  +0.94 }_{  -0.91}$ & $^{  +1.02 }_{  -1.12}$ & $^{  +0.54 }_{  -0.49}$ & $^{  +0.18 }_{  -0.24}$ & $^{  +0.10 }_{  -0.22}$ \\ [0.5mm] 
Closeby jets (JES) & $^{  -1.80 }_{  +1.59}$ & $^{  -0.47 }_{  +0.51}$ & $^{  +0.76 }_{  -0.85}$ & $^{  +1.03 }_{  -0.92}$ & $^{  +0.98 }_{  -0.86}$ & $^{  +1.14 }_{  -1.29}$ & $^{  +1.45 }_{  -1.68}$ \\ [0.5mm] 
Effective detector NP set 1 (JES) & $^{  -1.54 }_{  +1.13}$ & $^{  -0.54 }_{  +0.61}$ & $^{  +0.68 }_{  -0.62}$ & $^{  +1.07 }_{  -1.07}$ & $^{  +1.15 }_{  -0.94}$ & $^{  +1.11 }_{  -0.81}$ & $^{  +1.35 }_{  -0.38}$ \\ [0.5mm] 
Effective detector NP set 2 (JES) & $^{  -0.18 }_{  +0.09}$ & $^{  -0.09 }_{  +0.04}$ & $^{  +0.03 }_{  -0.07}$ & $^{  +0.27 }_{  -0.05}$ & $^{  +0.19 }_{  +0.07}$ & $^{  +0.12 }_{  -0.17}$ & $^{  +0.21 }_{  -0.29}$ \\ [0.5mm] 
Effective mixed NP set 1 (JES) & $^{  -0.05 }_{  +0.01}$ & $^{  -0.05 }_{  +0.06}$ & $^{  +0.02 }_{  -0.05}$ & $^{  +0.08 }_{  -0.12}$ & $^{  +0.01 }_{  -0.11}$ & $^{  +0.18 }_{  +0.08}$ & $^{  +0.73 }_{  +0.33}$ \\ [0.5mm] 
Effective mixed NP set 2 (JES) & $^{  -0.07 }_{  -0.03}$ & $^{  -0.01 }_{  +0.03}$ & $^{  +0.05 }_{  -0.08}$ & $^{  -0.05 }_{  -0.07}$ & $^{  +0.06 }_{  -0.02}$ & $^{  +0.03 }_{  +0.15}$ & $^{  +0.18 }_{  +0.78}$ \\ [0.5mm] 
Effective model NP set 1 (JES) & $^{  +0.18 }_{  +0.10}$ & $^{  -0.05 }_{  +0.09}$ & $^{  -0.07 }_{  -0.41}$ & $^{  +0.15 }_{  -0.14}$ & $^{  +0.11 }_{  +0.59}$ & $^{  -0.74 }_{  +1.04}$ & $^{  -1.49 }_{  +1.60}$ \\ [0.5mm] 
Effective model NP set 2 (JES) & $^{  -0.54 }_{  +0.58}$ & $^{  -0.28 }_{  +0.16}$ & $^{  +0.09 }_{  -0.18}$ & $^{  +0.56 }_{  -0.42}$ & $^{  +0.59 }_{  -0.52}$ & $^{  +0.71 }_{  -0.53}$ & $^{  +1.17 }_{  -0.57}$ \\ [0.5mm] 
Effective model NP set 3 (JES) & $^{  +0.63 }_{  -0.79}$ & $^{  +0.20 }_{  -0.28}$ & $^{  -0.30 }_{  +0.19}$ & $^{  -0.48 }_{  +0.67}$ & $^{  -0.45 }_{  +0.81}$ & $^{  -0.43 }_{  +0.73}$ & $^{  -0.33 }_{  +0.77}$ \\ [0.5mm] 
Effective model NP set 4 (JES) & $^{  -0.16 }_{  +0.16}$ & $^{  -0.04 }_{  -0.02}$ & $^{  +0.04 }_{  -0.07}$ & $^{  +0.06 }_{  +0.03}$ & $^{  +0.18 }_{  -0.08}$ & $^{  +0.09 }_{  -0.04}$ & $^{  +0.20 }_{  +0.12}$ \\ [0.5mm] 
Effective stat. NP set 1 (JES) & $^{  +0.48 }_{  -0.64}$ & $^{  +0.11 }_{  -0.11}$ & $^{  -0.21 }_{  -0.02}$ & $^{  -0.19 }_{  +0.41}$ & $^{  -0.31 }_{  +0.69}$ & $^{  -0.89 }_{  +1.01}$ & $^{  -1.19 }_{  +1.51}$ \\ [0.5mm] 
Effective stat. NP set 2 (JES) & $^{  -0.23 }_{  +0.19}$ & $^{  -0.04 }_{  +0.04}$ & $^{  +0.04 }_{  -0.09}$ & $^{  +0.11 }_{  -0.10}$ & $^{  +0.10 }_{  -0.12}$ & $^{  +0.18 }_{  -0.16}$ & $^{  +0.43 }_{  -0.00}$ \\ [0.5mm] 
Effective stat. NP set 3 (JES) & $^{  -0.42 }_{  +0.36}$ & $^{  -0.15 }_{  +0.13}$ & $^{  +0.20 }_{  -0.18}$ & $^{  +0.35 }_{  -0.29}$ & $^{  +0.35 }_{  -0.31}$ & $^{  +0.26 }_{  -0.34}$ & $^{  +0.41 }_{  -0.12}$ \\ [0.5mm] 
$\eta$-intercalibration (JES) & $^{  -0.77 }_{  +0.67}$ & $^{  -0.17 }_{  +0.33}$ & $^{  +0.41 }_{  -0.47}$ & $^{  +0.50 }_{  -0.68}$ & $^{  +0.31 }_{  -0.13}$ & $^{  -0.15 }_{  +0.06}$ & $^{  -0.44 }_{  +0.16}$ \\ [0.5mm] 
$\eta$-intercalibration statistics (JES) & $^{  -0.13 }_{  -0.20}$ & $^{  -0.10 }_{  +0.02}$ & $^{  +0.06 }_{  +0.02}$ & $^{  +0.23 }_{  +0.04}$ & $^{  +0.27 }_{  +0.07}$ & $^{  +0.00 }_{  +0.22}$ & $^{  +0.12 }_{  +0.58}$ \\ [0.5mm] 
Flavor composition (JES) & $^{  +0.03 }_{  +0.10}$ & $^{  -0.02 }_{  +0.13}$ & $^{  -0.04 }_{  -0.10}$ & $^{  -0.01 }_{  -0.20}$ & $^{  +0.22 }_{  -0.24}$ & $^{  +0.21 }_{  -0.21}$ & $^{  +0.39 }_{  +0.05}$ \\ [0.5mm] 
Flavor response (JES) & $^{  +0.37 }_{  -0.76}$ & $^{  +0.14 }_{  -0.00}$ & $^{  -0.14 }_{  +0.17}$ & $^{  -0.29 }_{  +0.34}$ & $^{  -0.22 }_{  +0.54}$ & $^{  -0.55 }_{  +0.61}$ & $^{  -0.60 }_{  +0.77}$ \\ [0.5mm] 
Pile-up offset $\mu$ (JES) & $^{  -0.09 }_{  +0.33}$ & $^{  -0.11 }_{  +0.02}$ & $^{  -0.13 }_{  -0.19}$ & $^{  +0.20 }_{  -0.25}$ & $^{  +0.56 }_{  +0.19}$ & $^{  +0.31 }_{  +0.15}$ & $^{  +0.07 }_{  +0.64}$ \\ [0.5mm] 
Pile-up offset $N_{\rm PV}$ (JES) & $^{  +0.05 }_{  -0.28}$ & $^{  +0.19 }_{  -0.01}$ & $^{  -0.17 }_{  +0.04}$ & $^{  -0.17 }_{  +0.03}$ & $^{  -0.11 }_{  +0.19}$ & $^{  -0.03 }_{  +0.31}$ & $^{  +0.23 }_{  +0.62}$ \\ [0.5mm] 
Relative non-closure MC (JES) & $^{  -0.10 }_{  +0.09}$ & $^{  -0.09 }_{  +0.06}$ & $^{  +0.02 }_{  -0.17}$ & $^{  +0.16 }_{  -0.01}$ & $^{  +0.22 }_{  +0.03}$ & $^{  +0.11 }_{  -0.04}$ & $^{  +0.18 }_{  +0.19}$ \\ [0.5mm] 
Single particle high-\pt{} (JES) & $^{  +0.03 }_{  +0.03}$ & $^{  -0.02 }_{  -0.02}$ & $^{  -0.01 }_{  -0.02}$ & $^{  +0.03 }_{  +0.03}$ & $^{  +0.02 }_{  +0.03}$ & $^{  -0.00 }_{  -0.00}$ & $^{  +0.00 }_{  +0.01}$ \\ [0.5mm] 
JES uncertainty in background & $^{  -0.17 }_{  +0.25}$ & $^{  +0.17 }_{  -0.20}$ & $^{  +0.31 }_{  -0.19}$ & $^{  -0.57 }_{  +0.09}$ & $^{  -1.14 }_{  +0.37}$ & $^{  -0.36 }_{  +0.57}$ & $^{  +0.77 }_{  +1.48}$ \\ [0.5mm] 
Jet energy resolution & $^{  +0.52 }_{  -0.52}$ & $^{  -0.13 }_{  +0.13}$ & $^{  -0.51 }_{  +0.51}$ & $^{  +0.11 }_{  -0.11}$ & $^{  +0.51 }_{  -0.51}$ & $^{  +0.28 }_{  -0.28}$ & $^{  +0.71 }_{  -0.71}$ \\ [0.5mm] 
Jet reconstruction efficiency & $^{  +0.14 }_{  -0.14}$ & $^{  -0.04 }_{  +0.04}$ & $^{  -0.06 }_{  +0.06}$ & $^{  +0.04 }_{  -0.04}$ & $^{  -0.00 }_{  +0.00}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.16 }_{  +0.16}$ \\ [0.5mm] 
$b$-quark tagging efficiency & $^{  -1.38 }_{  +1.10}$ & $^{  -0.71 }_{  +0.53}$ & $^{  +0.29 }_{  -0.30}$ & $^{  +1.28 }_{  -1.04}$ & $^{  +2.09 }_{  -1.53}$ & $^{  +2.58 }_{  -1.60}$ & $^{  +3.00 }_{  -1.63}$ \\ [0.5mm] 
$c$-quark tagging efficiency & $^{  -0.02 }_{  +0.01}$ & $^{  +0.01 }_{  -0.01}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.01 }_{  +0.02}$ & $^{  -0.08 }_{  +0.08}$ & $^{  -0.11 }_{  +0.12}$ & $^{  -0.21 }_{  +0.21}$ \\ [0.5mm] 
Light-jet tagging efficiency & $^{  +0.25 }_{  -0.24}$ & $^{  +0.03 }_{  -0.02}$ & $^{  -0.12 }_{  +0.12}$ & $^{  -0.13 }_{  +0.12}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.00 }_{  +0.01}$ & $^{  +0.18 }_{  -0.15}$ \\ [0.5mm] 
$e$ energy resolution & $^{  -0.05 }_{  +0.06}$ & $^{  +0.02 }_{  +0.01}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.09 }_{  -0.02}$ & $^{  -0.09 }_{  -0.01}$ & $^{  +0.11 }_{  +0.02}$ & $^{  +0.32 }_{  -0.07}$ \\ [0.5mm] 
$e$ energy scale & $^{  +0.07 }_{  -0.04}$ & $^{  +0.08 }_{  -0.04}$ & $^{  -0.01 }_{  +0.03}$ & $^{  -0.15 }_{  +0.03}$ & $^{  -0.14 }_{  -0.02}$ & $^{  -0.30 }_{  +0.07}$ & $^{  -0.36 }_{  +0.10}$ \\ [0.5mm] 
$\mu$ ID momentum resolution & $^{  +0.38 }_{  +0.37}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.21 }_{  -0.27}$ & $^{  -0.06 }_{  -0.05}$ & $^{  +0.02 }_{  +0.01}$ & $^{  +0.02 }_{  +0.03}$ & $^{  +0.16 }_{  +0.19}$ \\ [0.5mm] 
$\mu$ MS momentum resolution & $^{  +0.40 }_{  +0.31}$ & $^{  +0.06 }_{  -0.00}$ & $^{  -0.28 }_{  -0.09}$ & $^{  -0.15 }_{  -0.10}$ & $^{  -0.10 }_{  -0.12}$ & $^{  +0.04 }_{  -0.07}$ & $^{  +0.30 }_{  +0.30}$ \\ [0.5mm] 
$\mu$ momentum scale & $^{  +0.19 }_{  -0.19}$ & $^{  -0.03 }_{  +0.03}$ & $^{  -0.11 }_{  +0.11}$ & $^{  -0.05 }_{  +0.05}$ & $^{  +0.15 }_{  -0.15}$ & $^{  +0.14 }_{  -0.14}$ & $^{  +0.28 }_{  -0.28}$ \\ [0.5mm] 
$\ell$ ID efficiency & $^{  +0.06 }_{  -0.06}$ & $^{  +0.04 }_{  -0.04}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.07 }_{  +0.07}$ & $^{  -0.08 }_{  +0.09}$ & $^{  -0.11 }_{  +0.11}$ & $^{  -0.09 }_{  +0.09}$ \\ [0.5mm] 
$\ell$ reconstruction efficiency & $^{  +0.02 }_{  -0.02}$ & $^{  +0.01 }_{  -0.01}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.01 }_{  +0.01}$ \\ [0.5mm] 
$\ell$ trigger efficiency & $^{  +0.05 }_{  -0.05}$ & $^{  +0.02 }_{  -0.02}$ & $^{  -0.02 }_{  +0.02}$ & $^{  -0.04 }_{  +0.04}$ & $^{  -0.05 }_{  +0.05}$ & $^{  -0.06 }_{  +0.06}$ & $^{  -0.07 }_{  +0.07}$ \\ [0.5mm] 
\Etmiss{} cell-out & $^{  -0.05 }_{  +0.34}$ & $^{  -0.03 }_{  +0.03}$ & $^{  +0.18 }_{  -0.28}$ & $^{  +0.13 }_{  -0.21}$ & $^{  -0.23 }_{  +0.25}$ & $^{  -0.38 }_{  +0.23}$ & $^{  +0.18 }_{  +0.27}$ \\ [0.5mm] 
\Etmiss{} pile-up & $^{  -0.03 }_{  +0.47}$ & $^{  -0.02 }_{  +0.02}$ & $^{  +0.05 }_{  -0.41}$ & $^{  -0.08 }_{  -0.23}$ & $^{  +0.24 }_{  +0.29}$ & $^{  +0.53 }_{  +0.42}$ & $^{  +0.62 }_{  +0.61}$ \\ [0.5mm] 
MC generator & $^{  -1.90 }_{  +1.90}$ & $^{  +0.32 }_{  -0.32}$ & $^{  +1.02 }_{  -1.02}$ & $^{  +0.95 }_{  -0.95}$ & $^{  -0.55 }_{  +0.55}$ & $^{  -3.36 }_{  +3.36}$ & $^{  -9.06 }_{  +9.06}$ \\ [0.5mm] 
Fragmentation & $^{  -1.10 }_{  +1.10}$ & $^{  +0.42 }_{  -0.42}$ & $^{  +0.27 }_{  -0.27}$ & $^{  +0.06 }_{  -0.06}$ & $^{  -1.20 }_{  +1.20}$ & $^{  -1.55 }_{  +1.55}$ & $^{  +0.31 }_{  -0.31}$ \\ [0.5mm] 
IFSR & $^{  +2.75 }_{  -2.75}$ & $^{  +1.12 }_{  -1.12}$ & $^{  -1.18 }_{  +1.18}$ & $^{  -2.19 }_{  +2.19}$ & $^{  -2.18 }_{  +2.18}$ & $^{  -0.55 }_{  +0.55}$ & $^{  +0.71 }_{  -0.71}$ \\ [0.5mm] 
PDF & $^{  +0.13 }_{  -0.13}$ & $^{  +0.14 }_{  -0.14}$ & $^{  +0.03 }_{  -0.03}$ & $^{  -0.16 }_{  +0.16}$ & $^{  -0.43 }_{  +0.43}$ & $^{  -0.79 }_{  +0.79}$ & $^{  -0.78 }_{  +0.78}$ \\ [0.5mm] 
MC statistics & $^{  +1.00 }_{  -1.00}$ & $^{  +0.40 }_{  -0.40}$ & $^{  +0.68 }_{  -0.68}$ & $^{  +0.89 }_{  -0.89}$ & $^{  +1.06 }_{  -1.06}$ & $^{  +1.41 }_{  -1.41}$ & $^{  +2.56 }_{  -2.56}$ \\ [0.5mm] 
\Wboson+jets bb4 & $^{  +0.33 }_{  -0.34}$ & $^{  +0.05 }_{  -0.06}$ & $^{  -0.13 }_{  +0.11}$ & $^{  -0.08 }_{  +0.15}$ & $^{  -0.17 }_{  +0.22}$ & $^{  -0.33 }_{  +0.32}$ & $^{  -0.23 }_{  +0.39}$ \\ [0.5mm] 
\Wboson+jets bb5 & $^{  +0.33 }_{  +0.00}$ & $^{  +0.05 }_{  +0.01}$ & $^{  -0.13 }_{  +0.02}$ & $^{  -0.08 }_{  -0.07}$ & $^{  -0.17 }_{  -0.04}$ & $^{  -0.33 }_{  +0.02}$ & $^{  -0.23 }_{  -0.14}$ \\ [0.5mm] 
\Wboson+jets bbcc & $^{  -0.15 }_{  +0.14}$ & $^{  -0.06 }_{  +0.06}$ & $^{  +0.01 }_{  -0.01}$ & $^{  +0.24 }_{  -0.23}$ & $^{  +0.17 }_{  -0.17}$ & $^{  +0.02 }_{  -0.02}$ & $^{  +0.23 }_{  -0.24}$ \\ [0.5mm] 
\Wboson+jets bbccc & $^{  +1.05 }_{  -1.16}$ & $^{  +0.18 }_{  -0.19}$ & $^{  -0.36 }_{  +0.40}$ & $^{  -0.47 }_{  +0.51}$ & $^{  -0.64 }_{  +0.71}$ & $^{  -0.93 }_{  +0.99}$ & $^{  -1.00 }_{  +1.07}$ \\ [0.5mm] 
\Wboson+jets c4 & $^{  +0.61 }_{  -0.45}$ & $^{  +0.08 }_{  -0.08}$ & $^{  -0.21 }_{  +0.16}$ & $^{  -0.28 }_{  +0.23}$ & $^{  -0.34 }_{  +0.29}$ & $^{  -0.38 }_{  +0.29}$ & $^{  -0.45 }_{  +0.31}$ \\ [0.5mm] 
\Wboson+Jets c5 & $^{  +0.61 }_{  -0.22}$ & $^{  +0.08 }_{  -0.01}$ & $^{  -0.21 }_{  +0.07}$ & $^{  -0.28 }_{  +0.08}$ & $^{  -0.34 }_{  +0.08}$ & $^{  -0.38 }_{  +0.12}$ & $^{  -0.45 }_{  +0.18}$ \\ [0.5mm] 
\Wboson+jets charge asymmetry & $^{  +0.96 }_{  -1.11}$ & $^{  +0.13 }_{  -0.14}$ & $^{  -0.37 }_{  +0.43}$ & $^{  -0.44 }_{  +0.48}$ & $^{  -0.52 }_{  +0.58}$ & $^{  -0.65 }_{  +0.74}$ & $^{  -0.47 }_{  +0.54}$ \\ [0.5mm] 
Multijet normalization & $^{  +0.78 }_{  -0.80}$ & $^{  +0.37 }_{  -0.38}$ & $^{  -0.36 }_{  +0.37}$ & $^{  -0.88 }_{  +0.92}$ & $^{  -0.54 }_{  +0.56}$ & $^{  -0.09 }_{  +0.09}$ & $^{  +0.27 }_{  -0.29}$ \\ [0.5mm] 
Multijet shape & $^{  -0.09 }_{  -0.33}$ & $^{  -0.17 }_{  -0.07}$ & $^{  +0.08 }_{  +0.12}$ & $^{  +0.27 }_{  +0.31}$ & $^{  +0.10 }_{  +0.19}$ & $^{  -0.21 }_{  +0.12}$ & $^{  -0.14 }_{  -0.13}$ \\ [0.5mm] 
$Z+$jets background normalization & $^{  +0.42 }_{  -0.43}$ & $^{  +0.14 }_{  -0.14}$ & $^{  -0.18 }_{  +0.18}$ & $^{  -0.37 }_{  +0.37}$ & $^{  -0.34 }_{  +0.34}$ & $^{  -0.31 }_{  +0.31}$ & $^{  -0.29 }_{  +0.29}$ \\ [0.5mm] 
Dilepton background normalization & $^{  +0.18 }_{  -0.17}$ & $^{  +0.12 }_{  -0.11}$ & $^{  -0.01 }_{  +0.01}$ & $^{  -0.20 }_{  +0.19}$ & $^{  -0.36 }_{  +0.34}$ & $^{  -0.49 }_{  +0.46}$ & $^{  -0.52 }_{  +0.50}$ \\ [0.5mm] 
\hline
Channels BLUE weights  & (0.24 ,0.76) & (0.54 ,0.46) & (0.18 ,0.82) & (0.51 ,0.49) & (0.40 ,0.60) & (0.49 ,0.51) & (0.33 ,0.67) \\ [2mm] 
\hline
\end{tabular}}


==> relativeUncertaintiesInCombination_Tag1_Top2_lhood_Norm_grouped.tex <==

\noindent\makebox[\textwidth]{
\begin{tabular}{l c c c c c c c}
\hline
$\frac{1}{\sigma} \frac{\dsigma}{\dptt}$ Uncertainties [\%] $/$ Bins [GeV] &    [0,  50] &    [50, 100] &    [100, 150] &    [150, 200] &    [200, 250] &    [250, 350] &    [350, 800] \\ 
\hline
\hline
Jet energy scale & $^{+    3.3 }_{-    3.0}$ & $^{+    1.0 }_{-    1.1}$ & $\pm    1.6$ & $\pm    2.2$ & $^{+    2.3 }_{-    2.1}$ & $^{+    2.3 }_{-    2.5}$ & $^{+    3.4 }_{-    3.7}$ \\ [1mm] 
Jet energy resolution & $\pm    0.5$ & $\pm    0.1$ & $\pm    0.5$ & $\pm    0.1$ & $\pm    0.5$ & $\pm    0.3$ & $\pm    0.7$ \\ [1mm] 
Jet reconstruction efficiency & $\pm    0.1$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & $\pm    0.2$ \\ [1mm] 
$b$-quark tagging efficiency & $^{+    1.4 }_{-    1.1}$ & $^{+    0.7 }_{-    0.5}$ & $\pm    0.3$ & $^{+    1.3 }_{-    1.0}$ & $^{+    2.1 }_{-    1.5}$ & $^{+    2.6 }_{-    1.6}$ & $^{+    3.0 }_{-    1.6}$ \\ [1mm] 
$c$-quark tagging efficiency & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & ${\rm --}$ & $\pm    0.1$ & $\pm    0.2$ \\ [1mm] 
Light-jet tagging efficiency & $\pm    0.2$ & ${\rm --}$ & $\pm    0.1$ & $\pm    0.1$ & ${\rm --}$ & ${\rm --}$ & $^{+    0.2 }_{-    0.1}$ \\ [1mm] 
Lepton selection and scaling & $^{+    0.6 }_{-    0.5}$ & $\pm    0.1$ & $^{+    0.4 }_{-    0.3}$ & $^{+    0.3 }_{-    0.2}$ & $^{+    0.3 }_{-    0.2}$ & $^{+    0.4 }_{-    0.2}$ & $^{+    0.7 }_{-    0.5}$ \\ [1mm] 
\Etmiss{} cell-out & $^{\rm --}_{-    0.3}$ & ${\rm --}$ & $^{+    0.2 }_{-    0.3}$ & $^{+    0.1 }_{-    0.2}$ & $^{+    0.2 }_{-    0.3}$ & $^{+    0.4 }_{-    0.2}$ & $^{+    0.2 }_{-    0.3}$ \\ [1mm] 
\Etmiss{} pile-up & $^{\rm --}_{-    0.5}$ & ${\rm --}$ & $^{\rm --}_{-    0.4}$ & $^{\rm --}_{-    0.2}$ & $^{+    0.2 }_{-    0.3}$ & $^{+    0.5 }_{-    0.4}$ & $\pm    0.6$ \\ [1mm] 
MC generator & $\pm    1.9$ & $\pm    0.3$ & $\pm    1.0$ & $\pm    1.0$ & $\pm    0.5$ & $\pm    3.4$ & $\pm    9.1$ \\ [1mm] 
Fragmentation & $\pm    1.1$ & $\pm    0.4$ & $\pm    0.3$ & ${\rm --}$ & $\pm    1.2$ & $\pm    1.5$ & $\pm    0.3$ \\ [1mm] 
IFSR & $\pm    2.8$ & $\pm    1.1$ & $\pm    1.2$ & $\pm    2.2$ & $\pm    2.2$ & $\pm    0.5$ & $\pm    0.7$ \\ [1mm] 
PDF & $\pm    0.1$ & $\pm    0.1$ & ${\rm --}$ & $\pm    0.2$ & $\pm    0.4$ & $\pm    0.8$ & $\pm    0.8$ \\ [1mm] 
MC statistics & $\pm    1.0$ & $\pm    0.4$ & $\pm    0.7$ & $\pm    0.9$ & $\pm    1.1$ & $\pm    1.4$ & $\pm    2.6$ \\ [1mm] 
\Wboson+jets & $\pm    1.7$ & $\pm    0.3$ & $\pm    0.6$ & $\pm    0.8$ & $\pm    1.0$ & $\pm    1.3$ & $\pm    1.3$ \\ [1mm] 
Other backgrounds & $^{+    0.9 }_{-    1.0}$ & $\pm    0.4$ & $\pm    0.4$ & $^{+    1.0 }_{-    1.1}$ & $^{+    0.7 }_{-    0.8}$ & $\pm    0.6$ & $\pm    0.7$ \\ [1mm] 
\hline
\hline
 Statistical uncertainty  & $\pm$2.5 & $\pm$1.0 & $\pm$1.7 & $\pm$1.9 & $\pm$2.3 & $\pm$3.3 & $\pm$6.1 \\ [2mm] 
 Total systematic uncertainty  & $^{+    5.5 }_{-    5.3}$ & $^{+    1.9 }_{-    1.8}$ & $^{+    2.5 }_{-    2.6}$ & $\pm    3.8$ & $^{+    4.4 }_{-    4.1}$ & $^{+    5.6 }_{-    5.3}$ & $^{+   10.7 }_{-   10.5}$ \\ [2mm] 
\hline
%%%Channels BLUE weights  & (0.24 ,0.76) & (0.54 ,0.46) & (0.18 ,0.82) & (0.51 ,0.49) & (0.40 ,0.60) & (0.49 ,0.51) & (0.33 ,0.67) \\ [2mm] 
\hline
\hline
\end{tabular}}

